Blind Cyclic Prefix-based CFO Estimation in MIMO-OFDM Systems

Low-complexity estimation and correction of carrier frequency offset (CFO) are essential in orthogonal frequency division multiplexing (OFDM). In this paper, we propose a low-overhead blind CFO estimation technique based on cyclic prefix (CP), in multi-input multi-output (MIMO)-OFDM systems. We propose to use antenna diversity for CFO estimation. Given that the RF chains for all antenna elements at a communication node share the same clock, the carrier frequency offset (CFO) between two points may be estimated by using the combination of the received signal at all antennas. We improve our method by combining the antenna diversity with time diversity by considering the CP for multiple OFDM symbols. We provide a closed-form expression for CFO estimation and present algorithms that can considerably improve the CFO estimation performance at the expense of a linear increase in computational complexity. We validate the effectiveness of our estimation scheme via extensive numerical analysis.

==> UPA_Codebook.tex <==
\subsection{UPA Codebook Design Prolem}

Suppose an $M_h \times M_v$ UPA is placed at the $x-z$ plane, and let $M = M_h M_v$. Let the distance between the antennas that are placed parallel to $z$ axis, be $d_z$, and $d_x$ respectively. One can define,

\begin{align}
\mathbf{d}_{M_{a}}\left(\psi_{a}\right) = \left[1, e^{j \psi_{a}} \cdots e^{j\left(M_{a}-1\right) \psi_{a}}\right]^{T} \in \mathbb{C}^{M_{a}}
\end{align}
where, $\psi_{h}=\frac{2 \pi d_{x}}{\lambda} \sin \theta \cos \phi \text { and } \psi_{v}=\frac{2 \pi d_{z}}{\lambda} \sin \phi$, and $a$ takes value in the set $\{v, h\}$.  
The array response vector is then defined as 

\begin{align}
    \mathbf{d}_{M}\left(\psi_{v}, \psi_{h}\right) =
    \mathbf{d}_{M_{v}}\left(\psi_{v}\right) \otimes
    \mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \in \mathbb{C}^{M}
\end{align}
Let $\mathcal{B}_s$ be the angular range under cover in the $(\psi_h, \psi_v)$ domain. We have, 

\begin{equation}
    \mathcal{B}^\psi_{s} \doteq\left[-\psi_h^{\mathrm{B}}, \psi_h^{\mathrm{B}}\right) \times\left[-\psi_v^{\mathrm{B}}, \psi_v^{\mathrm{B}}\right)
\end{equation}

% \begin{equation}
%     \mathcal{B}_{s} \doteq \left[-\phi^{\mathrm{B}}, \phi^{\mathrm{B}}\right)
%     \times \left[-\theta^{\mathrm{B}}, \theta^{\mathrm{B}}\right) \label{range_angle}
% \end{equation}

% Notation $\psi^{p,q}_{h}[1:L_h,1 :L_v], \psi^{p,q}_{v}[1:L_v]$

Let us uniformly divide the angular range  into $Q=Q_{v} Q_{h}$ subregions. For each subregion we have, 

% $$ \mathcal{B}_{p, q} =  \omega_{\phi, p} \times \omega_{\theta, q}$$

% Let $\Delta_{\theta} =  2 \theta^{\mathrm{B}} / Q_{v}$, and $\Delta_\phi =  2 \phi^{\mathrm{B}} / Q_{h}$ be the length of each sub-interval along axis $\theta$, and $\phi$. We have $\omega_{\theta, q} = [\theta_{q-1}, \theta_q)$, and, $\omega_{\phi, p} = [\phi_{p-1},\phi_p)$ where  $\theta_q = -\theta^B + q\Delta_\theta$, and $\phi_p = -\phi^B + p\Delta_\phi$. 


$$ \mathcal{B}_{ p, q} \doteq \nu_{v}^{p, q} \times \nu_{h}^ {p, q}$$

% We can then write for each $v_{a, b}$, i.e the $b$-th sub-interval along axis $a$,

% \begin{equation}
%     \nu_{v, p} =-\psi_{a}^{\mathrm{B}}+(b-1)\Delta_{a}+\left[0, \Delta_{a}\right)
% \end{equation}

Define the reference gain at $(\psi_{h}, \psi_{v}) $ as, 

\begin{equation}
    G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) =\left|\left(\mathbf{d}_{M_{v}}\left(\psi_{v}\right)\otimes\mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \right)^{H} \mathbf{c}\right|^{2}
\end{equation}

It is straightforward to show that, 

\begin{equation}
    \int_{-\pi}^{\pi} \int_{-\pi}^{\pi} G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) d \psi_{v} d \psi_{h}={(2 \pi)^{2}}
\end{equation}

Therefore, for every interval $\mathcal{B}_{ p, q}$ we can derive the ideal gain expression as, 

\begin{equation}
    G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)=G_{p,q} \mathds{1}_{\mathcal{B}^\psi_{p, q}}\left(\psi_{v}, \psi_{h}\right)
\end{equation}

where $G_{q,p} = \frac{(2\pi)^2}{\delta_{p,q}}$, where $\delta_{p,q}$ is the area of the interval $\mathcal{B}^\psi_{p,q}$. We can write $\delta_{p,q} = \delta_v\delta_h = (\frac{2\psi^B_v}{Q_v})(\frac{2\psi^B_h}{Q_h})$. Therefore, We define the codebook design problem under the UPA structure as follows. 
% where $G_{q,p} = \frac{(2\pi)^2}{\delta^{p,q}_h\delta^p_v}$, $\delta^p_v = \psi^p_v - \psi^{p-1}_v $, and $\delta^{q, p}_h = \psi^{q,p}_h - \psi^{q-1, p}_h $. Also, let us define $\delta_{q,p} = \delta^{q, p}_h\delta^p_v$. 



\begin{align}
& \c^{opt}_{p, q} = \nonumber\\&\underset{\c, \|\c\|=1}{\arg \min } \iint_{\mathcal{B}_{s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \label{init_opt}
\end{align}

By partitioning the range of $(\psi_h, \psi_v)$ into the pre-defined intervals, we can rewrite the optimization problem as follows, 

\begin{align}
& \c^{opt}_{p, q} = \underset{\c, \|\c\|=1}{\arg \min }\nonumber\\& \sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\iint_{\mathcal{B}^{\psi}_{r,s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \nonumber\\&
 = \underset{L_h, L_v \rightarrow \infty}{\lim}\sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\sum_{l_v =1}^{L_v}\sum_{l_h =1}^{L_h}\frac{\delta_v\delta_h}{L_hL_v}\nonumber\\&
\left|G_{p, q}^{\text {ideal }}\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_h]\right)-G\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_h], \c\right)\right| \label{alternative_opt}
\end{align}
where, 

\begin{align}
    &\psi^{r,s}_v[l_v] = \psi^{r-1, s}_v + l_v\frac{\delta_v}{L_v}\nonumber\\
    &\psi^{r,s}_h[l_h] = \psi^{r, s-1}_h + l_h\frac{\delta_h}{L_h}
\end{align}

We can rewrite the optimization problem \eqref{alternative_opt} as, 

\begin{align}
    \c_{p,q}^{opt}=\arg \min _{\c, \|\c\|=1} \underset{L_h, L_v \rightarrow \infty}{\lim}\frac{1}{L_hL_v}\left\|\mathbf{G}^{\text {ideal }}_{p,q}-\mathbf{G}(\c)\right\|
\end{align}


where, 

\begin{align}
    \mathbf{G}(\c) =& \delta_v\delta_h\left[G\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1], \c\right) \cdots \right. \nonumber\\ &\left. G\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{h}\right], \c\right)\right]^{T} 
\end{align}

and, 

\begin{align}
    \mathbf{G}^{\text {ideal }}_{ p, q} =& \delta_v\delta_h\left[G^{\text {ideal }}_{ p, q}\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1] \right) \cdots \right. \nonumber\\ &\left. G^{\text {ideal }}_{ p, q}\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{h}\right]\right)\right]^{T} 
\end{align}


% \begin{align}
%      &\mathbf{G}^{\text {ideal }}_{ q, p}= \nonumber\\&\left[{\delta_{1,1}} G^{\text {ideal }} _{q, p}\left(\psi^{1}_{h}[1], \psi^{1}_{v}[1], \c\right) \ldots {\delta_{Q_h, Q_v}}G^{\text {ideal }} _{q, p}\left(\psi^{Q_h}_{h}[L_h], \psi^{Q_v}_{v}[L_v], \c\right)\right]^{T} 
% \end{align}


Note that we can write, 

\begin{align}
    \mathbf{G}^{\text{ideal }}_{p,q} = \delta_v\delta_h\frac{{(2\pi)}^2}{\delta_v\delta_h} \left(\e_{p,q} \otimes \mathbf{1}_{L, 1}\right)
\end{align}


with $\mathbf{e}_{p,q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $(p,q)$-th axis among $Q$ ones. 








Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, we can write: 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


\begin{align}
\mathbf{G}^{\text {ideal }}_{p,q} &={{(2\pi)}^2}\left(\mathbf{e}_{p,q} \otimes(\mathbf{g} \odot \mathbf{g}^{*})\right) \nonumber\\
&=\left({{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)\right) \odot \left({{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)\right)^* \label{g_id_q_equivalent}
\end{align}

Also, note that we can write, 

% \begin{align}
%     \mathbf{G}(\c)=\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right) \odot\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right)^{*}
% \end{align}
\begin{align}
    \mathbf{G}(\c)=\left(\D^H \c\right) \odot\left(\D^H \c\right)^{*}
\end{align}

\noindent where, $\D^H = \sqrt{\delta_v\delta_h}(\mathbf{D}_{v}^{H} \otimes \mathbf{D}_{h}^{H})$, and for $a \in \{v,h\}$, we have, 

\begin{align}
\mathbf{D}_{a} &=\left[\mathbf{D}_{a, 1}, \cdots, \mathbf{D}_{a, Q_{a}}\right] \in \mathbb{C}^{M_{a} \times L_{a} Q_{a}} \\
\mathbf{D}_{a, b} &=\left[\mathbf{d}_{M_{a}}\left(\psi_{a}^{b}[1]\right), \cdots, \mathbf{d}_{M_{a}}\left(\psi_{a}^{b}\left[L_{a}\right]\right)\right] \in \mathbb{C}^{M_{a} \times L_{a}}
\end{align}




% where 

% \begin{align}
%     \D = \left[D^{1,1}_{vh}, \cdots, D^{Q_v,Q_h}_{vh}\right] \in \mathbb{C}^{M_vM_h\times L_vL_hQ_vQ_h}
% \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% &\mathbf{D}_{h, q}(\chi) =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1], \chi \right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right], \chi \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% &\mathbf{D}_{vh, p,q} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}[1]), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}\left[L_{v}\right]) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% \mathbf{D}^{p,q}_{h}(\ell) =&\sqrt{\delta_v^{p}\delta^{p,q,\ell}_h}\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}[\ell][1] \right), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}\left[\ell] [L_{h} \right] \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}, 
% \end{align}

% \begin{align}
%     \mathbf{D}_{vh}^{p,q} =&\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}[1]\right) \otimes \mathbf{D}_{h}^{p,q}(1), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h}^{p,q}(L_{v}) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}

\begin{problem}
Given an equal-gain vector $\g_{p,q} \in \mathbb{C}^L$, $(p,q) \in \{(1,1), \cdots, (Q_v, Q_h)\}$, find vector $\c_{p,q} \in \mathbb{C}^{M_t}$ such that
\begin{align}
&\c_{p,q}=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|{{2\pi}}\left(\mathbf{e}_{p,q} \otimes \mathbf{g}\right)- \D^H \c\right\|^{2} \label{obj_func}
\end{align}
\label{main_problem_UPA}
\end{problem}


Note that the solution to problem \ref{main_problem_UPA} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
 \begin{align}
 {\c}^{(L)}_{p,q} &= {{{2\pi}}}(\D \D^H)^{-1} \D  \left(\mathbf{e}_{p,q} \otimes \mathbf{g}_{p,q}\right) \nonumber\\& =\sigma \D_{p,q}\mathbf{g}_{p,q}
\end{align}
where $\sigma = \frac{2\pi \sqrt{\delta_{v}\delta_{h}}}{LQ\delta_{v}\delta_{h}} = \frac{2\pi}{LQ\sqrt{\delta_v\delta_h}}$, noting that it holds that, 

Noting that it holds that, 

\begin{align}
    (\D\D^H) = \left(L\sum_{(p,q)= (1,1)}^{(Q_h, Q_v)}\sum_{(l_v,l_h)= (1,1)}^{(L_h, L_v)} \delta_{v}\delta_{h}\right)\I_{M_t}
\end{align}

\begin{problem}
Find equal-gain $\g_{p,q} \in \mathbb{C}^L$, $(p,q) = (1,1), \ldots, (Q_h, Q_v)$, such that
\begin{equation}
 \g_{q,p} = \underset{\g}{\arg\min }\left\| abs(\D^H \c_{p,q})- {2\pi} abs(\mathbf{e}_{p,q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
\end{equation} 
where $abs(.)$ denotes the element-wise absolute value of a vector.
\label{g_problem}
\end{problem}


\begin{proposition}
The minimizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha_v^{\eta (L_v -1)}\alpha_h^{\eta (L_h -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha_v = e^{j(\frac{\eta_v}{L_v})}$ and $\alpha_h = e^{j(\frac{\eta_h}{L_h})}$. \label{proposiiton_g}
\end{proposition}

 \begin{align}
     {\c_{p,q}}^{(L)} & = \sigma \sum_{(l_v, l_h)=(1,1)}^{(L_v, L_h)}g_{p,q, l}\mathbf{d}_{M_t}\left(\psi^{p}_{v}[l_v], \psi^{q}_{h}[l_h]\right)  \nonumber\\
     & = \sigma \sum_{l=1}^L g_{q,p,l}\left[{\begin{array}{ccc}
     1 &\cdots & e^{j\phi_{p,q}^{M_v-1, M_h-1}}\\
     \end{array}}\right]^T   
    %  \nonumber\\& = \left[{\begin{array}{ccc}
    %  \sigma\sum_{l=1}^L g_{q, p, l}& \cdots & \sigma\sum_{l=1}^L g_{q,p, l}e^{j\left((M_h-1)\psi^q_{h}[l] + (M_v-1)\psi^p_{v}[l]\right)}\\
    %  \end{array}}\right]^T
\end{align}

where $ \phi_{p,q}^{m_v, m_h} = \left( m_v\psi^{p}_{v}[l_v] + m_h\psi^{q}_{h}[l_h]\right)$. We can then write 

\begin{align}
    c_{p,q, m_v, m_h} &= \nonumber\\& \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} g_{p,q, l_v, l_h}e^{j\phi_{p,q}^{M_v-1, M_h-1}}
\end{align}


\begin{align}
    c_{p,q, m_v, m_h} &=  \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} g_{p,q, l_v, l_h}\nonumber \\&e^{j\left(m_v(\psi^{p-1}_{v}+l_v\frac{\delta_v}{L_v})+ m_h(\psi^{q-1}_{h} + l_h\frac{\delta_h}{L_h}) \right)}
\end{align}


\begin{align}
    c_{p,q, m_v, m_h} =&  \frac{2\pi}{Q}e^{j\phi_{p-1, q-1}^{m_v, m_h}}
    \left(\frac{1}{L_v}\lim_{ L_v\rightarrow \infty} \sum_{l_v=1}^{L_v} e^{j\frac{\eta_v+ m_v\delta_v}{L_v} l_v}\right) \nonumber\\&
    \left(\frac{1}{L_h}\lim_{ L_h\rightarrow \infty} \sum_{l_h=1}^{L_h} e^{j\frac{\eta_h+ m_h\delta_h}{L_h} l_h}\right)
\end{align}

\begin{align}
    c_{p,q, m_v, m_h} &=  \frac{2\pi}{Q}e^{j\phi_{p-1, q-1}^{m_v, m_h}}
    \int_{0}^{1} e^{j\xi_v x}dx\int_{0}^{1} e^{j\xi_h x}dx \nonumber\\&
    = \frac{2\pi}{Q}e^{j(\phi_{p-1, q-1}^{m_v, m_h}+ \frac{\xi_v+\xi_h}{2})} sinc(\frac{\xi_v}{2\pi})sinc(\frac{\xi_h}{2\pi})
\end{align}

with $\xi_a = {\delta_a}{m_a} + \eta_a$, where $a\in \{v,h\}$. 
% Therefore, it. holds that, 

% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi}) 
% \end{align}

==> composite.tex <==
\subsection{Composite Codebook Design Problem}

Let us define a \textit{composite beam} $\omega_k$ as a union of multiple disjoint, possibly non-neighboring beams $\nu_{q} \text { for } q \in \mathcal{Q} = \left\{1, \cdots, Q\right\}$. Let $\mathcal{C'}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{K}\right\}$ be the codebook corresponding to the composite problem.

% $$\bigcup_{k = 1}^{2^{B'}}{\omega_k} = [-\pi, \pi], \quad \text{and} \quad \omega_k \cap \omega_l = \emptyset, \quad \forall k\neq l.$$

Moreover, define for each composite beam $\omega_k$ the set $\mathcal{W}_k \subseteq \mathcal{Q}$ to be the set of indices of the single beams that form $\omega_k$. i.e. $\mathcal{W}_k = \{q \in \mathcal{Q}: v_q \subseteq \omega_k\}$. 
For any codeword $\c$, it holds that, 

\begin{equation}
    \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\|\mathbf{c}\|^{2}=2 \pi
\end{equation}
We have then for the ideal gain corresponding to  each codeword $\textbf{c}_k$, 

\begin{align}
&\int_{-\pi}^{\pi} G_{\text {ideal }, k}(\psi) d \psi =\int_{\omega_{k}} t d \psi+\int_{[-\pi, \pi] \backslash \omega_{k}} 0 d \psi \nonumber\\
&= \sum_{q \in {\mathcal{W}_k}}{\int_{\nu_{q}} t d \psi} = \sum_{q \in \mathcal{W}_k}\delta_q t=2 \pi \label{composite}
\end{align}

Therefore, $t = \frac{2 \pi}{\Delta_k}$, where $\Delta_k = \sum_{q \in \mathcal{W}_k}\delta_q$. It follows that, 

\begin{equation}
    G_{\text {ideal }, k}(\psi)=\frac{2 \pi}{\Delta_k} \mathds{1}_{\omega_{k}}(\psi), \quad \psi \in[-\pi, \pi] \label{composite_ideal_gain}
\end{equation}

The new MSE problem for the $k$-th codeword can therefore be written as follows.



\begin{align}
\c_k^{opt} &=\underset{\c, \|\c\|=1}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, k}(\psi)-G(\psi, \c)\right| d \psi 
\end{align}




By uniformly sampling on the range of   we can rewrite
the optimization problem as follows,

\begin{align}
    \c_k^{opt} &= \nonumber \\&\underset{\c, \|\c\|=1}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \delta_p\sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \c\right)\right|}{L}\right]\label{composite_MSE}
\end{align}

 where, for $q = 1 \ldots Q$, 
 $$\delta_q = \psi_{q}-\psi_{q-1}, \quad \psi_{q, \ell}=\psi_{q-1}+\frac{\delta_q(\ell-0.5)}{L} $$

We can rewrite equation \eqref{composite_MSE} as follows, 

\begin{align}
 &\c_k^{opt} = \underset{\c,  \|\c\|=1}{\arg \min } \lim_{L\rightarrow \infty}\frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\c)\right\| \label{init_opt}
 \end{align}
 
 where,  $$\mathbf{G}(\c)=\left[{\delta_1} G\left(\psi_{1,1}, \c\right) \ldots {\delta_{Q}}G\left(\psi_{Q, L}, \c\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

and, 
$$ \mathbf{G}_{\text {ideal }, k}=\left[{\delta_1} G_{\text {ideal }, k}\left(\psi_{1,1}\right) \ldots {\delta_{Q}}G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$


Note that it holds that 

\begin{equation}
    \mathbf{G}_{\text {ideal },k}=\sum_{q \in \mathcal{W}_k}\delta_q\frac{2\pi}{\Delta_k}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right) \label{ideal}
\end{equation}

with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, for a suitable choice of $\g$ we can write: 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


\begin{align}
\mathbf{G}_{\text {ideal }, k} &= \sum_{q \in \mathcal{W}_k}\gamma_q\left(\mathbf{e}_{q} \otimes\left(\mathbf{g} \odot \mathbf{g}^{*}\right)\right) \nonumber\\
&=\sum_{q \in \mathcal{W}_k}\left(\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right) \odot\left(\sqrt{{\gamma_q}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right)^{*} \nonumber\\
&=\left(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
\end{align}




















% \begin{align}
% \left(\mathbf{F}_{k}, \mathbf{v}_{k}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \sum_{p=1}^{Q} \sum_{\ell=1}^{L}\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2} \nonumber\\
% &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min }\lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\mathbf{F} \mathbf{v})\right\|_{2}^{2} \label{init_opt}
% \end{align}

% where,  $$\mathbf{G}(\mathbf{F} \mathbf{v})=\left[G\left(\psi_{1,1}, \mathbf{F} \mathbf{v}\right) \cdots G\left(\psi_{Q, L}, \mathbf{F} \mathbf{v}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% and, 
% $$ \mathbf{G}_{\text {ideal }, k}=\left[G_{\text {ideal }, k}\left(\psi_{1,1}\right) \cdots G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% Note that we can write using the definition of $\mathcal{W}_k$ that, 

% $$G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)=\left\{\begin{array}{ll}
% \frac{Q}{|\mathcal{W}_k| M_{t}}, & p \in \mathcal{W}_k \\
% 0, & p \notin \mathcal{W}_k 
% \end{array},\right.$$

% Or in the matrix form, 

% \begin{align}
%     &\mathbf{G}_{\text {ideal }, k}=\frac{Q}{|\mathcal{W}_k| M_{t}}\left((\bigoplus_{q \in \mathcal{W}_k}{\mathbf{e}_{q}}) \otimes \mathbf{1}_{L, 1}\right)  \nonumber \\ 
%     & = \sum_{q \in \mathcal{W}_k}{\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right)} \label{G_ideal_k}
% \end{align}

% with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any $\mathbf{g} \in \mathcal{G}_L$, where, 

% $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$



% Therefore, equation \eqref{G_ideal_k} can be rewritten as:
% \begin{align}
% &\mathbf{G}_{\text {ideal }, k} = \sum_{q \in \mathcal{W}_k}\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g}_q \odot \mathbf{g}_q^{*}\right)\right) \nonumber\\
% &=\sum_{q \in \mathcal{W}_k}\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right) \odot\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \nonumber\\
% &=\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
% \end{align}

% where $\sigma = \sqrt{\frac{Q}{|\mathcal{W}_k|M_{t}}}$. 

Similarly, it is straightforward to observe,


\begin{align}
\mathbf{G}(\c) &=\left(\mathbf{D}^{H} \c\right) \odot\left(\mathbf{D}^{H} \c\right)^{*} \label{dc}
\end{align}
where $\mathbf{D} =\left[\sqrt{\delta_1}\mathbf{D}_{1} \cdots \sqrt{\delta_{Q}}\mathbf{D}_{Q} \right] \in \mathbb{C}^{M_{t} \times L Q}$, and 
$\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}.$
 







% On the other hand note that $\mathbf{G}(\mathbf{F} \mathbf{v})$ can be written as,


% \begin{equation}
%     \mathbf{G}(\mathbf{F} \mathbf{v}) =\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right) \odot\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right)^{*}\label{dfv_decomp}
% \end{equation}

% where, 
% $$\mathbf{D} =\left[\mathbf{D}_{1} \cdots \mathbf{D}_{Q}\right] \in \mathbb{C}^{M_{t} \times L Q}$$

% and, $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}$. 

Comparing the expressions \eqref{init_opt}, \eqref{final_gik}, and \eqref{dc}, one can show that the optimal choice of $\c_q$ in \eqref{init_opt} is the solution to the following optimization problem for a proper choice of $\g_q$. 
\begin{problem}
Given an equal-gain vector $\g_q \in \mathbb{C}^L$, $q \in \{1, \cdots, Q\}$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
\begin{align}
&\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
\end{align}
\label{main_problem}
\end{problem}


However, we now need to find the optimal choice of $\g_q$ that minimizes the objective in \eqref{init_opt}. Using \eqref{final_gik}, and \eqref{dc}, we have the following optimization problem.
\begin{problem}
Find a set of equal-gain $\g_q \in \mathbb{C}^L$, i.e. $\mathcal{G}_k$ such that
\begin{equation}
 \mathcal{G}_k = \underset{\mathcal{G}}{\arg\min }\left\| abs(\D^H \c_q)- abs(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\mathbf{e}_{q} \otimes \mathbf{g}_q))\right\|^{2} \label{g_final_eq}
\end{equation} 
where $\mathcal{G}_k = \{\g_q| q \in \mathcal{W}_k\}$, and $abs(.)$ denotes the element-wise absolute value of a vector.
\label{g_problem}
\end{problem}

Hence, the codebook design for a system with full-digital beamforming capability is found by solving Problem~\ref{main_problem} for proper choice of $\g_q$ obtained as a solution to Problem ~\ref{g_problem}. The codebook for Hybrid beamforming, is then found as
\begin{align}
    \underset{\mathbf{F}_{q},\mathbf{v}_{q}}{\arg\min } \|\mathbf{F}_{q}\mathbf{v}_{q} - \c_q\|^2
\end{align}
where the columns of $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ are equal-gain vectors and $\v_q \in \mathbb{C}^{N_{RF}}$. The solution may be obtained using simple, yet effective suboptimal algorithm such as orthogonal matching pursuit (OMP) \cite{love15}\cite{noh17}\cite{Hussain17}. In the next section we continue with the solution of Problem~\ref{main_problem}, and~\ref{g_problem}.





% Comparing the expressions in equations \eqref{final_gik}, and, \eqref{dc}, a perfect solution to the optimization problem in \eqref{init_opt}, could be a pair $\textbf{(F, v)}$, for which the following equality holds.  



% \begin{align}
%     \mathbf{D}^{H} \mathbf{F} \mathbf{v}=\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right) \label{potential_answer}
% \end{align}

% However, we have that $M_t > N_{RF}$ and therefore, the matrix $\textbf{D}^H \textbf{F}$ may not be full-rank, resulting in the RHS of equation \eqref{potential_answer} being in the null space of LHS. Therefore, given some $\g_q \in \mathcal{G}_L$ we formulate the following two-step optimization problem to search for $\textbf{(F, v)}$ that gets as close as possible to the desired value. 

% \begin{problem}

% a) For all $q \in \{1, \cdots, Q\}$, given $\g_q \in \mathcal{G}_L$, find the unit-norm vector $\c_q \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c^{|\g_q}_q=\underset{\c}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)- \mathbf{D}^{H} \c\right\|_{2}^{2} \label{obj_func}
% \end{align}

% \noindent
% b) For every given $\c_q$, find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_RF}$ that satisfy $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ the condition $\f_n \in \mathcal{B}_{M_t}$ as in equation \eqref{f_constant_gain}. 

% \begin{align}
%     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% \end{align}

% \end{problem}



Note that the solution to problem \ref{main_problem} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
 \begin{align}
& {\c}^{(L)}_k = \sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\D \D^H)^{-1} \D  \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
& {\c}^{(L)}_k = \sum_{q \in \mathcal{W}_k}\sigma_q \D_q\g_q \label{c_final_eq}
\end{align}
where $\sigma_q = \frac{\sqrt{ 2\pi \delta_q \frac{\delta_q}{\Delta_k}}}{L \sum_{p=1}^{2^B}\delta_p} = \frac{\delta_q}{L\sqrt{2\pi\Delta_k}}$, noting that it holds that, 

% $$\mathbf{D D}^{H}=\left({L \sum_{p=1}^{2^B}\delta_p}\right) \mathbf{I}_{M_{t}}$$.
% % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 


Using \eqref{c_final_eq}, equation \eqref{g_final_eq} can now be rewritten as, 

\begin{align}
 &\mathcal{G}_k = \underset{\mathcal{G}}{\arg\min } \nonumber
 \\&\left\| abs(\D^H \D\sum_{q \in \mathcal{W}_k}\sigma_q(\mathbf{e}_{q} \otimes \mathbf{g}_q))-abs(\sum_{q \in \mathcal{W}_k}\sqrt{\gamma_q}(\mathbf{e}_{q} \otimes \mathbf{g}_q))\right\|^{2} \label{g_simple_final_eq}
\end{align} 

% where $\sigma' = \frac{1}{2\pi L}$. We will state the following theorem without formal proof.
\begin{proposition}
The maximizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha = e^{j(\frac{\delta_q}{L})}$. \label{proposiiton_g}
\end{proposition}

An analytical closed form solution for $\c_q$ can be found as follows. We have, 
 \begin{align}
     {\c_k}^{(L)} & = \sum_{q \in \mathcal{W}_k} \sigma_q \left(\sum_{l=1}^{L}g_{q, l}\mathbf{d}_{M_t}(\psi_{q, l})\right)  \nonumber\\
     & = \sum_{q \in \mathcal{W}_k} \left(\sum_{l=1}^L \sigma_qg_q^{(l)}\left[{\begin{array}{ccc}
     1 &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^T \right)  \nonumber\\
     & = \sum_{q \in \mathcal{W}_k} \sigma_q \left[{\begin{array}{ccc}
     \sum_{l=1}^L g_{q, l}& \cdots & \sum_{l=1}^L g_{q, l}e^{j(M_t-1)\psi_{q, l}}\\
     \end{array}}\right]^T 
\end{align}

 
Let us write, 

\begin{equation}
    \c_k^{(L)} = \sum_{q \in \mathcal{W}_k} \c_q^{(L)}
\end{equation}

where, 

\begin{equation}
{\c_q}^{(L)}  = \sigma_q \sum_{l=1}^{L}g_{q, l}\mathbf{d}_{M_t}(\psi_{q, l})
\end{equation}


Choosing $\g_q$ as in proposition \ref{proposiiton_g},  the $m$-th element of the vector ${\c}_q = \lim_{L\rightarrow \infty}{\c_q}^{(L)} $, i.e. $c_{q,m}$, is given by 

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_{q, l} e^{j(m\psi_{q, l+1})}
\end{equation}

% With a choice of $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % $\alpha = e^j(\frac{2\pi}{L2^B})$
% $\alpha = e^{j(\frac{\delta_q}{L})}$ and suitable $\eta$ (to be determined later), we can write


% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{L2^B})}
% \end{equation}

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_{q, l} e^{jm(\psi_{q-1}+\frac{\delta_q(\ell+0.5)}{L})}
\end{equation}

% After some basic manipulations we get, 
\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}\lim_{L\rightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5\delta_q}{L})} 
\end{equation}


\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
\end{equation}

\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
\end{equation}


\begin{equation}
    c_{q,m} = \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{L2^B}x}dx
\end{equation}


\begin{align}
 c_{q,m} &= \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{jm\psi_{q-1}} \int_{0}^{1} e^{j\xi x}dx \nonumber \\
 &= \frac{\delta_q}{\sqrt{2\pi}\Delta_k}e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}) \label{final_g}
\end{align}

where $\xi = \delta_q (\eta +m )$.


% \begin{equation}
%     c_{q,m} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% \end{equation}

% \begin{equation}
%     c_{q,m} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% \end{equation}

% \begin{equation}
%     c_{q,m} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}) \label{final_g}
% \end{equation}






% Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
%  \begin{align}
% & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% \end{align}
% Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% \begin{equation}
%     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% \end{equation}

% We aim to find $\g_q$ such that

% \begin{align}
% & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% \end{align}

% is minimized.

% % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% \begin{align}
%      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
%      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
%      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
%      \end{array}}\right]^T  = \nonumber\\
%      & \left[{\begin{array}{cccc}
%      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
%      \end{array}}\right]^T
%  \end{align}
 
 

%  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% \end{equation}

% With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % $\alpha = e^j(\frac{2\pi}{LQ})$
% $\alpha = e^j(\frac{\psi_{q}-\psi_{q-1}}{L})$ and suitable $\eta$ (to be determined later), we can write


% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % \end{equation}

% \begin{equation}
%     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% \end{equation}


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % \end{equation}


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% \end{equation}

% where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% \begin{equation}
%     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% \end{equation}

% \begin{equation}
%     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% \end{equation}

% where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.
















% We first optimize for $\alpha$ by setting the derivative of \eqref{obj_func} to zero, to get: 

% $$\hat{\alpha}=\frac{\sum_{q \in \mathcal{W}_k}\sqrt{\frac{Q}{M_{t}}}(\mathbf{F} \mathbf{v})^{H} \mathbf{D}_{q} \mathbf{g}_q}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}}$$

% Replacing the value of $\alpha$ as above we get to the following optimization problem. 

% \begin{align}
% \left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max } \frac{\left|\sum_{q \in \mathcal{W}_k}\sqrt{\frac{2^{\mathbf{B}}}{M_{t}}}\left(\mathbf{D}_{q} \mathbf{g}_q\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}} \nonumber \\
% &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max }\left|\sum_{q \in \mathcal{W}_k}\left(\mathbf{D}_{q} \mathbf{g}\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}
% \end{align}


% \section{Codebook Design Problem Formulation}
% \label{sec: formulation}

% % Let $\mathbf{c} \doteq \mathbf{F} \mathbf{v} \in \mathbb{C}^{M_{t}}$ be the unit-norm transmit beam-forming codeword, where analog beamsteering matrix $\mathbf{F}=\left[\mathbf{f}_{1}, \cdots, \mathbf{f}_{N_{R F}}\right] \in \mathbb{C}^{M_{t} \times N_{R F}}$ contains $N_{RF}$ equal-gain analog beamsteering vectors $\mathbf{f}_{n}$ and the baseband beamforming vector $\mathbf{v} \in \mathbb{C}^{N_{R F}}$ is such that $\|\c\|_{2}=1$ holds. The equal-gain constraint holds if $\mathbf{f}_{n} \in \mathcal{B}_{M_{t}}$ for 

% % \begin{equation}
% %     \mathcal{B}_{M_{t}}=\left\{\mathbf{w} \in \mathbb{C}^{M_{t}}:\left(\mathbf{w} \mathbf{w}^{H}\right)_{\ell, \ell}=1 / M_{t}, 1 \leq \ell \leq M_{t}\right\}
% %     \label{f_constant_gain}
% % \end{equation}

% % Let $\mathcal{C}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{Q}\right\}$ be the codebook with codewords taking value as $\mathbf{c}_{q}=\mathbf{F}_{q} \mathbf{v}_{q}$. Consider a half-wavelength uniform linear array (ULA) of antennas as in the previous subsection, i.e. $d = \frac{\lambda}{2}$, with an array response vector as in \eqref{array_factor}.

% % % %$$\mathbf{d}_{M_{t}}(\psi)=\frac{1}{\sqrt{M_{t}}}\left[1 e^{j \psi} \cdots e^{j\left(M_{t}-1\right) \psi}\right]^{T} \in \mathbb{C}^{M_{t}}$$
% % % $$\mathbf{d}_{M_{t}}(\psi)=\left[1, e^{j \psi}, \cdots, e^{j\left(M_{t}-1\right) \psi}\right]^{T} \in \mathbb{C}^{M_{t}}$$

%  For convenience, in this section, we will drop the index \emph{ula} from the expression of the array factor $\d_{ula, M_t}(\psi)$ and gain $G^{ula}(\psi, \mathbf{c})$.  Before presenting the formulation of the codebook design problem, we introduce some new notations. We divide the angular range of $\theta \in [-\pi, 0]$  into equal-length beams $\omega_{q} \text { for } q \in\left\{1, \cdots, Q\right\}$. i.e. 
% $$
% \begin{aligned}
% \omega_{q} &=\left[\theta_{q-1}, \theta_{q}\right) ,& \theta_{q}= -\pi+ \frac{ \pi}{Q} q
% \end{aligned}
% $$

% % Further we introduce the change of variable $\psi = \frac{2 \pi d}{\lambda} \cos(\theta)$ where $\psi \in [-\pi, \pi]$. For $d = \frac{\lambda}{2}$,

% Corresponding to $\omega_q$ intervals, there exists $\nu_q$ ranges with respect to $\psi$ such that, 

% $$
% \begin{aligned}
% \nu_{q} &=\left[\psi_{q-1}, \psi_{q}\right), & \psi_q = -\pi\cos(\frac{\pi}{Q}q)
% \end{aligned}
% $$


% Under the reference gain as in \eqref{reference gain} and using Parseval's theorem \cite{parseval}, we will have:
% % and assuming $|\c| = 1$
% \begin{equation}
% \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\left\| \mathbf{c}\right\|^{2}=2 \pi\label{parseval}
% \end{equation}

% Let  $G_{\text {ideal }, q}(\psi)$ denote the desired ideal gain which is supposed to be constant on $\nu_q$ and zero otherwise. It must hold that, 
% % \begin{equation}
% % \int_{-\pi}^{\pi} G(\psi, \mathbf{c}) d \psi=2 \pi\left\|\frac{1}{\sqrt{M_{t}}} \mathbf{c}\right\|_{2}^{2}=\frac{2 \pi}{M_{t}}    \label{parseval}
% % \end{equation}





% \begin{align}
% &\int_{-\pi}^{\pi} G_{\text {ideal }, q}(\psi) d \psi =\int_{\nu_{q}} t d \psi+\int_{[-\pi, \pi] \backslash \nu_{q}} 0 d \psi \nonumber\\
% &=(\psi_q - \psi_{q-1}) t={2 \pi} \label{plain}
% \end{align}

% which in turn will give: 

% \begin{equation}
%     G_{\text {ideal }, q}(\psi)=\frac{2\pi}{(\psi_q - \psi_{q-1})} \mathds{1}_{\nu_{q}}(\psi), \quad \psi \in[-\pi, \pi] \label{ideal_gain}
% \end{equation}

% We aim to design the codebooks so as to mimic the ideal gain computed in equation \eqref{ideal_gain}. Therefore, the plain codebook design problem is formulated as a minimization of a MSE as follows: 


% % \begin{align}
% % &\left(\mathbf{F}_{\text {opt }, q}, \mathbf{v}_{\mathrm{opt}, q}\right) \nonumber \\&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, q}(\psi)-G(\psi, \mathbf{F} \mathbf{v})\right|^{2} d \psi
% % \end{align}

% \begin{align}
% &\c_q^{opt}=\underset{\c, \|\c\|=1}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, q}(\psi)-G(\psi, \c)\right| d \psi
% \label{composite_MSE}
% \end{align}

% By uniformly sampling on the range of $\psi$ we can rewrite the optimization problem as follows, 
% \begin{align}
%     &\underset{\c, \|\c\|=1}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \delta_p \sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, q}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \c \right)\right|}{L}\right]\label{equivalent_MSE}
% \end{align}

%  where for $q = 1 \ldots Q$, 
%  $$\delta_q = \psi_{q}-\psi_{q-1}, \quad \psi_{q, \ell}=\psi_{q-1}+\frac{\delta_q(\ell-0.5)}{L} $$

 
%  We can write equation \eqref{equivalent_MSE}, as 
%  \begin{align}
%  &\c_q^{opt} = \underset{\c,  \|\c\|=1}{\arg \min } \lim_{L\rightarrow \infty}\frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, q}-\mathbf{G}(\c)\right\| \label{init_opt}
%  \end{align}
 
%  where,  $$\mathbf{G}(\c)=\left[{\delta_1} G\left(\psi_{1,1}, \c\right) \ldots {\delta_{Q}}G\left(\psi_{Q, L}, \c\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% and, 
% $$ \mathbf{G}_{\text {ideal }, q}=\left[{\delta_1} G_{\text {ideal }, q}\left(\psi_{1,1}\right) \ldots {\delta_{Q}}G_{\text {ideal }, q}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% Note that it holds that 

% \begin{equation}
%     \mathbf{G}_{\text {ideal }, q}={2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right) \label{ideal}
% \end{equation}

% with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, for a suitable choice of $\g$ we can write: 

% % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


% \begin{align}
% \mathbf{G}_{\text {ideal }, q} &={2\pi}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g} \odot \mathbf{g}^{*}\right)\right) \nonumber\\
% &=\left(\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right) \odot\left(\sqrt{{2\pi}}\left(\mathbf{e}_{q} \otimes \mathbf{g}\right)\right)^{*} \label{g_id_q_equivalent}
% \end{align}


% Similarly, it is straightforward to observe,


% \begin{align}
% \mathbf{G}(\c) &=\left(\mathbf{D}^{H} \c\right) \odot\left(\mathbf{D}^{H} \c\right)^{*} \label{dc}
% \end{align}
% where $\mathbf{D} =\left[\sqrt{\delta_1}\mathbf{D}_{1} \cdots \sqrt{\delta_{Q}}\mathbf{D}_{Q} \right] \in \mathbb{C}^{M_{t} \times L Q}$, and 
% $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}.$
 

% % Comparing the expressions in equations \eqref{g_id_q_equivalent} and \eqref{dc},  we formulate the following two-step optimization for the codebook design problem for hybrid beamforming, presented below as \textit{Problem \ref{main_problem}}. Given a suitable $\g_q$, in the first step, we search for a unit-norm codeword $\c_q$ for fully-digital beamforming, and in the second step we find a suitable pair $(\F_q, \v_q)$ to complete the hybrid beamforming codebook design.  

 

% % \begin{problem}

% % a) For all $q \in \{1, \cdots, Q\}$, given equal-gain $\g_q \in \mathbb{C}^L$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
% % \begin{align}
% % &\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\longrightarrow \infty} \left\|\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
% % \end{align}

% % \vspace{2mm}
% % \noindent
% % b) Find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_{RF}}$ that solve $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ subject to the equal-gain condition on the columns of $\F_q$. 

% % % \begin{align}
% % %     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% % % \end{align}
% % \label{main_problem}
% % \end{problem}

% % The solution to the last problem provides the optimal codebook designed for hybrid beamforming under a ULA structure, given the choice of $\g_q$. Note that we were initially trying to solve the optimization problem in equation \eqref{init_opt}. In light of modifications \eqref{g_id_q_equivalent}, and \eqref{dc}, the quantity to be minimized in the limit of equation \eqref{init_opt} can be written as follows,

% % \begin{align}
% %     & \left\|\mathbf{G}_{\text {ideal }, q}-\mathbf{G}(\c)\right\| = \left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\| \label{g_init}
% % \end{align}
% % where $abs(.)$ denotes the element-wise absolute value of a vector.

% % Equation \eqref{g_init} reveals the central role of the vector $\g_q$ in minimizing the MSE in equation \eqref{init_opt}. In fact, the choice of $\g_q$ has to be optimized in a way that norm in \eqref{g_init} is minimized; i.e. the result gain designed by codebook $\c_q$ gets as close as possible to the ideal gain. To optimize the choice of $\g_q$, we formulate the following optimization problem, presented as \textit{Problem \ref{g_problem}}.

% % \begin{problem}
% % For all $q = 1, \ldots, Q$, find equal-gain $\g_q \in \mathbb{C}^L$ such that

% % \begin{equation}
% %  \g_q = \underset{\g}{\arg\min }\left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% % \end{equation} 

% % \label{g_problem}
% % \end{problem}

% % In the next session we propose our approach to solve problems \ref{main_problem} and \ref{g_problem}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comparing the expressions \eqref{init_opt}, \eqref{g_id_q_equivalent}, and \eqref{dc}, one can show that the optimal choice of $\c_q$ in \eqref{init_opt} is the solution to the following optimization problem for a proper choice of $\g_q$. 
% \begin{problem}
% Given an equal-gain vector $\g_q \in \mathbb{C}^L$, $q \in \{1, \cdots, Q\}$, find vector $\c_q \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c_q=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\longrightarrow \infty} \left\|\sqrt{2\pi}\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)- \mathbf{D}^{H} \c\right\|^{2} \label{obj_func}
% \end{align}
% \label{main_problem}
% \end{problem}
% However, we now need to find the optimal choice of $\g_q$ that minimizes the objective in \eqref{init_opt}. Using \eqref{g_id_q_equivalent}, and \eqref{dc}, we have the following optimization problem.
% \begin{problem}
% Find equal-gain $\g_q \in \mathbb{C}^L$, $q = 1, \ldots, Q$, such that
% \begin{equation}
%  \g_q = \underset{\g}{\arg\min }\left\| abs(\D^H \c_q)- \sqrt{2\pi} abs(\mathbf{e}_{q} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% \end{equation} 
% where $abs(.)$ denotes the element-wise absolute value of a vector.
% \label{g_problem}
% \end{problem}

% Hence, the codebook design for a system with full-digital beamforming capability is found by solving Problem~\ref{main_problem} for proper choice of $\g_q$ obtained as a solution to Problem ~\ref{g_problem}. The codebook for Hybrid beamforming, is then found as
% \begin{align}
%     \underset{\mathbf{F}_{q},\mathbf{v}_{q}}{\arg\min } \|\mathbf{F}_{q}\mathbf{v}_{q} - \c_q\|^2
% \end{align}
% where the columns of $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ are equal-gain vectors and $\v_q \in \mathbb{C}^{N_{RF}}$. The solution may be obtained using simple, yet effective suboptimal algorithm such as orthogonal matching pursuit (OMP) \cite{love15}\cite{noh17}\cite{Hussain17}. In the next section we continue with the solution of Problem~\ref{main_problem}, and~\ref{g_problem}.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
% %  \begin{align}
% % & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% % \end{align}
% % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% % \begin{equation}
% %     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% % \end{equation}

% % We aim to find $\g_q$ such that

% % \begin{align}
% % & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% % \end{align}

% % is minimized.

% % % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% % We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% % \begin{align}
% %      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
% %      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
% %      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
% %      \end{array}}\right]^T  = \nonumber\\
% %      & \left[{\begin{array}{cccc}
% %      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
% %      \end{array}}\right]^T
% %  \end{align}
 
 

% %  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% % \end{equation}

% % With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % % $\alpha = e^j(\frac{2\pi}{LQ})$
% % $\alpha = e^{j(\frac{\psi_{q}-\psi_{q-1}}{L})}$ and suitable $\eta$ (to be determined later), we can write


% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % % \end{equation}

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% % \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % % \end{equation}


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% % \end{equation}

% % where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% % \begin{equation}
% %     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% % \end{equation}

% % \begin{equation}
% %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% % \end{equation}

% % where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.

% % \subsection{Twin-ULA Setting}

% % We start from problem \eqref{main_problem}, and particularly, equation \eqref{obj_func}. Let $\{\s_m\}_{m =0}^{M_t -1}$ denote the columns of $D^H$. We can write: 

% % \begin{align}
% % &\s_m c_q^{(m)} + \s_{m+M_t/2} c_q^{(m+M_t/2)} \nonumber\\
% % &= \s_m (c_q^{(m)} + e^{-j \frac{2\pi d_y}{\lambda} \sin(\theta)} c_q^{(m+M_t/2)}) \nonumber\\
% % & \approx \s_m \Tilde{c}_q^{(m)}, \quad  m = 0 \ldots \frac{M_t}{2}-1\end{align}

% % where we define 
% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = c_q^{(m)} + e^{-j \frac{2\pi d_y}{\lambda} \sin(\theta^{(m)}_q)} c_q^{(m+M_t/2)} \label{c_defn}
% % \end{equation}

% % with $\theta_{q-1}\leq\theta^{(m)}_q \leq \theta_{q}$ being a constant value.  

% % Therefore, the solution to part $(a)$ of problem \eqref{main_problem}, under the twin-ULA setup can be expressed as:

% %  \begin{align}
% % & \Tilde{\c}_q = (\Tilde{\D} \Tilde{\D}^H)^{-1} \Tilde{\D} \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % & \Tilde{\c}_q =  \sigma' \Tilde{\D} \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \Tilde{\D}_q\g_q
% % \end{align}

% % where it holds that $\Tilde{\D} \Tilde{\D}^H = \I_{\frac{M_t}{2}}$, and


% % $$\Tilde{\D}_{q}=\left[\d_{\frac{M_{t}}{2}}\left(\psi_{q, 1}\right) \cdots \d_{\frac{M_{t}}{2}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{\frac{M_{t}}{2} \times L}$$

% % In other words, one can approximately think of the codebook design problem over a twin ULA of $M_t$ antennas, as such a problem over a ULA of size $\frac{M_t}{2}$.

% % Following the approach in the previous subsection, we can infer, 

% % \begin{equation}
% %     \Tilde{c}_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi}), \quad m = 0 \ldots \frac{M_t}{2} -1
% %     \label{twin_c_result}
% % \end{equation}

% % Having $d_y = \frac{\lambda}{3}$, equating equations \eqref{c_defn}, and \eqref{twin_c_result}, by further assuming $c_q^{(m + \frac{M_t}{2})} = e^{j\beta_m} c_q^{(m)}$, after basic operations we get: 

% % \begin{equation}
% %     c_q^{(m)} = \frac{e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})}{1+ e^{-j(\frac{2\pi}{3}\sin(\theta_q^{(m)}) + \beta_m)}}
% % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = \frac{e^{j(m\psi_{q-1} + \frac{\xi}{2} +\frac{\pi}{3}\sin(\theta_q^{(m)})+\frac{\beta_m}{2}) sinc(\frac{\xi}{2\pi})}}{2\cos(\frac{\pi}{3}\sin(\theta_q^{(m)}) + \frac{\beta_m}{2})}
% % % \end{equation}

% % Therefore, for each codeword entry $c_q^{(m)}$, it remains to pick $\beta_m$ and $\theta_q^{(m)}$. We relax this decision by setting $\beta_m = \beta$, and $\theta_q^{(m)} = \theta_q$, $ m = 1 \ldots M_t$. Next we explicitly right the expression for the reference gain as $G(\theta, \c_{twin}) = \left|\d_{twin, M_{t}}^{H}(\theta) \c_{twin}\right|^{2}$ where 

% % \begin{align}
% %     &\d_{twin, M_{t}}(\theta) = \left[\d_{\frac{M_{t}}{2}}^{T}(\theta), e^{j(\frac{2\pi}{3}\sin(\theta))}\d_{\frac{M_{t}}{2}}^{T}(\theta)\right]^T\\
% %     & \c_{twin} = \left[\c^T_{twin, \frac{M_t}{2}}, e^{j\beta}\c^T_{twin, \frac{M_t}{2}}\right]^T
% % \end{align}

% % We can  therefore write, 

% % \begin{align}
% %     G(\theta, \c_{twin}) &= \left|\d_{\frac{M_{t}}{2}}^{H}(\theta)\c_{twin, \frac{M_t}{2}} (1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))})\right|^2\nonumber\\
% %     & = \left|\d_{\frac{M_{t}}{2}}^{H}(\theta)\c\right|^2 \left| \frac{1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))}}{1 + e^{-j(\beta+\frac{2\pi}{3}\sin(\theta))}}\right|^2
% % \end{align}

% % Further define 
% % $$ L(\theta) = \left| \frac{1 + e^{j(\beta-\frac{2\pi}{3}\sin(\theta))}}{1 + e^{-j(\beta+\frac{2\pi}{3}\sin(\theta))}}\right|$$
% % The last equation consists of two parts, the first part being the gain corresponding to a ULA of size $\frac{M_t}{2}$ and the second part being  $L^2(\theta)$. For any $\omega_q = \left[\theta_{q-1}, \theta_{q}\right)$, there exist a $\omega'_q \doteq \left(- \theta_{q}, -\theta_{q-1}\right]$. The gain of a ULA is symmetric over $\omega_q$, and $\omega'_q$ by definition. However utilizing a twin ULA we wish to suppress the gain over $\omega'_q$ as much as we can and contribute to the gain over $\omega_q$ for each codeword $c_q, \quad q = 1\ldots Q$. To this end, we define the \emph{isolation factor} $\mu$ as follows,

% % \begin{align}
% %     \mu = \underset{\omega_q}{\int}{\frac{L(-\theta)}{L(\theta)}} d\theta
% % \end{align}
% %  to denote the level of isolation between each $\omega_q$ and its counterpart.
 
 















% % % \subsection{Composite Codebook Design Problem}

% % % Let us define a \textit{composite beam} $\omega_k$ as a union of multiple disjoint, possibly non-neighboring beams $\nu_{q} \text { for } q \in \mathcal{Q} = \left\{1, \cdots, Q\right\}$. Let $\mathcal{C'}=\left\{\mathbf{c}_{1}, \cdots, \mathbf{c}_{K}\right\}$ be the codebook corresponding to the composite problem.

% % % % $$\bigcup_{k = 1}^{2^{B'}}{\omega_k} = [-\pi, \pi], \quad \text{and} \quad \omega_k \cap \omega_l = \emptyset, \quad \forall k\neq l.$$

% % % Moreover, define for each composite beam $\omega_k$ the set $\mathcal{W}_k \subseteq \mathcal{Q}$ to be the set of indices of the single beams that form $\omega_k$. i.e. $\mathcal{W}_k = \{q \in \mathcal{Q}: v_q \subseteq \omega_k\}$. 
% % % We have then for the new ideal gain for each new codeword $\textbf{c}_k$, 

% % % \begin{align}
% % % &\int_{-\pi}^{\pi} G_{\text {ideal }, k}(\psi) d \psi =\int_{\omega_{k}} t' d \psi+\int_{[-\pi, \pi] \backslash \omega_{k}} 0 d \psi \nonumber\\
% % % &= \sum_{q \in {\mathcal{W}_k}}{\int_{\nu_{q}} t' d \psi} = |\mathcal{W}_k|\frac{2 \pi}{Q} t'=\frac{2 \pi}{M_{t}} \label{composite}
% % % \end{align}

% % % Therefore, $t' = \frac{Q}{|\mathcal{W}_k| M_t}$. It follows that, 

% % % \begin{equation}
% % %     G_{\text {ideal }, k}(\psi)=\frac{Q}{|\mathcal{W}_k| M_{t}} \mathds{1}_{\omega_{k}}(\psi), \quad \psi \in[-\pi, \pi] \label{composite_ideal_gain}
% % % \end{equation}

% % % The new MSE problem for the $k$-th codeword can therefore be written as follows.

% % % \begin{align}
% % % &\left(\mathbf{F}_{\text {opt }, k}, \mathbf{v}_{\mathrm{opt}, k}\right) \nonumber \\&=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \int_{-\pi}^{\pi}\left|G_{\text {ideal }, k}(\psi)-G(\psi, \mathbf{F} \mathbf{v})\right|^{2} d \psi \nonumber \\&= \underset{\mathbf{F}, \mathbf{v}}{\arg \min }\left[\lim _{L \rightarrow \infty} \sum_{p=1}^{Q} \sum_{\ell=1}^{L} \frac{\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2}}{L Q / 2 \pi}\right]\label{composite_MSE}
% % % \end{align}


% % % \begin{align}
% % % \left(\mathbf{F}_{k}, \mathbf{v}_{k}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min } \sum_{p=1}^{Q} \sum_{\ell=1}^{L}\left|G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)-G\left(\psi_{p, \ell}, \mathbf{F} \mathbf{v}\right)\right|^{2} \nonumber\\
% % % &=\underset{\mathbf{F}, \mathbf{v}}{\arg \min }\lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\mathbf{G}_{\text {ideal }, k}-\mathbf{G}(\mathbf{F} \mathbf{v})\right\|_{2}^{2} \label{init_opt}
% % % \end{align}

% % % where,  $$\mathbf{G}(\mathbf{F} \mathbf{v})=\left[G\left(\psi_{1,1}, \mathbf{F} \mathbf{v}\right) \cdots G\left(\psi_{Q, L}, \mathbf{F} \mathbf{v}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% % % and, 
% % % $$ \mathbf{G}_{\text {ideal }, k}=\left[G_{\text {ideal }, k}\left(\psi_{1,1}\right) \cdots G_{\text {ideal }, k}\left(\psi_{Q, L}\right)\right]^{T} \in \mathbb{Z}^{L Q}$$

% % % Note that we can write using the definition of $\mathcal{W}_k$ that, 

% % % $$G_{\text {ideal }, k}\left(\psi_{p, \ell}\right)=\left\{\begin{array}{ll}
% % % \frac{Q}{|\mathcal{W}_k| M_{t}}, & p \in \mathcal{W}_k \\
% % % 0, & p \notin \mathcal{W}_k 
% % % \end{array},\right.$$

% % % Or in the matrix form, 

% % % \begin{align}
% % %     &\mathbf{G}_{\text {ideal }, k}=\frac{Q}{|\mathcal{W}_k| M_{t}}\left((\bigoplus_{q \in \mathcal{W}_k}{\mathbf{e}_{q}}) \otimes \mathbf{1}_{L, 1}\right)  \nonumber \\ 
% % %     & = \sum_{q \in \mathcal{W}_k}{\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes \mathbf{1}_{L, 1}\right)} \label{G_ideal_k}
% % % \end{align}

% % % with $\mathbf{e}_{q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $q$-th axis among $Q$ ones. Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any $\mathbf{g} \in \mathcal{G}_L$, where, 

% % % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$



% % % Therefore, equation \eqref{G_ideal_k} can be rewritten as:
% % % \begin{align}
% % % &\mathbf{G}_{\text {ideal }, k} = \sum_{q \in \mathcal{W}_k}\frac{Q}{|\mathcal{W}_k| M_{t}}\left(\mathbf{e}_{q} \otimes\left(\mathbf{g}_q \odot \mathbf{g}_q^{*}\right)\right) \nonumber\\
% % % &=\sum_{q \in \mathcal{W}_k}\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right) \odot\left(\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \nonumber\\
% % % &=\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)  \odot \left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)^{*} \label{final_gik}
% % % \end{align}

% % % where $\sigma = \sqrt{\frac{Q}{|\mathcal{W}_k|M_{t}}}$. 
% % % On the other hand note that $\mathbf{G}(\mathbf{F} \mathbf{v})$ can be written as,


% % % \begin{equation}
% % %     \mathbf{G}(\mathbf{F} \mathbf{v}) =\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right) \odot\left(\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right)^{*}\label{dfv_decomp}
% % % \end{equation}

% % % where, 
% % % $$\mathbf{D} =\left[\mathbf{D}_{1} \cdots \mathbf{D}_{Q}\right] \in \mathbb{C}^{M_{t} \times L Q}$$

% % % and, $\mathbf{D}_{q}=\left[\mathbf{d}_{M_{t}}\left(\psi_{q, 1}\right) \cdots \mathbf{d}_{M_{t}}\left(\psi_{q, L}\right)\right] \in \mathbb{C}^{M_{t} \times L}$. 

% % % Comparing the expressions in equations \eqref{final_gik}, and, \eqref{dfv_decomp}, a perfect solution to the optimization problem in \eqref{init_opt}, could be a pair $\textbf{(F, v)}$, for which the following equality holds.  



% % % \begin{align}
% % %     \mathbf{D}^{H} \mathbf{F} \mathbf{v}=\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right) \label{potential_answer}
% % % \end{align}

% % % However, we have that $M_t > N_{RF}$ and therefore, the matrix $\textbf{D}^H \textbf{F}$ may not be full-rank, resulting in the RHS of equation \eqref{potential_answer} being in the null space of LHS. Therefore, given some $\g_q \in \mathcal{G}_L$ we formulate the following two-step optimization problem to search for $\textbf{(F, v)}$ that gets as close as possible to the desired value. 

% % % \begin{problem}

% % % a) For all $q \in \{1, \cdots, Q\}$, given $\g_q \in \mathcal{G}_L$, find the unit-norm vector $\c_q \in \mathbb{C}^{M_t}$ such that
% % % \begin{align}
% % % &\c^{|\g_q}_q=\underset{\c}{\arg \min } \lim_{L\longrightarrow \infty} \frac{1}{L}\left\|\left(\sum_{q \in \mathcal{W}_k}\sigma\left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)\right)- \mathbf{D}^{H} \c\right\|_{2}^{2} \label{obj_func}
% % % \end{align}

% % % \noindent
% % % b) For every given $\c_q$, find $\F_q \in \mathbb{C}^{M_t \times N_{RF}}$ , and $\v_q \in \mathbb{C}^{N_RF}$ that satisfy $\mathbf{F}_{q}\mathbf{v}_{q} = \c_q$ the condition $\f_n \in \mathcal{B}_{M_t}$ as in equation \eqref{f_constant_gain}. 

% % % % \begin{align}
% % % %     \mathbf{F}_{\mid \g_q}\mathbf{v}_{\mid \g_q} = \c_q
% % % % \end{align}

% % % \end{problem}

% % % Note that the solution to part \textit{(a)} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity.
% % %  \begin{align}
% % % & \Tilde{\c}^{(L)}_q = (\D \D^H)^{-1} \D \sigma \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) \\
% % % & \Tilde{\c}^{(L)}_q =  \sigma' \D \left(\mathbf{e}_q \otimes \mathbf{g}_q\right) = \sigma' \D_q\g_q
% % % \end{align}
% % % Dividing by $\|\Tilde{\c}^{(L)}_q\|$ and taking the limit as L goes to infinity we will find the optimal $\c_q$. i.e. 

% % % \begin{equation}
% % %     \c_q = \lim_{L\longrightarrow \infty} \frac{\Tilde{\c}^{(L)}_q}{L\|\Tilde{\c}^{(L)}_q\|}
% % % \end{equation}

% % % We aim to find $\g_q$ such that

% % % \begin{align}
% % % & \left\| abs(\D^H \gamma' \D_q \mathbf{g}_q)- abs(\gamma \left(\mathbf{e}_{q} \otimes \mathbf{g}_q\right)) \right\|_{2}^{2}
% % % \end{align}

% % % is minimized.

% % % % Is it possible to show that $\g_q$ is independent of $q$ (assume regular scenario)? If true, i.e., $\g_q = \g$ we have

% % % We will provide a suboptimal structure for the choice of $\g$. Let us assume $\g_q = \g, $  for all $ q \in \{1, \cdots, Q\}$. Then we can write
% % % \begin{align}
% % %      &\Tilde{\c_q}^{(L)} = D_q\mathbf{g} = \sum_{l=1}^{L}g_l\mathbf{d}_{M_t}(\psi_{q, l})  \nonumber\\
% % %      & = \sum_{l=1}^L g_l\left[{\begin{array}{cccc}
% % %      1& e^{j\psi_{q, l}} &\cdots & e^{j(M_t-1)\psi_{q, l}}\\
% % %      \end{array}}\right]^T  = \nonumber\\
% % %      & \left[{\begin{array}{cccc}
% % %      \sum_{l=1}^L g_l& \sum_{l=1}^L g_le^{j\psi_{q, l}} &\cdots & \sum_{l=1}^L g_le^{j(M_t-1)\psi_{q, l}}\\
% % %      \end{array}}\right]^T
% % %  \end{align}
 
 

% % %  We have for the $m$-th element of the vector $\Tilde{\c}_q$, i.e. $\Tilde{c}^{(m)}_q$  for $ 0 \leq m \leq M_t-1$

% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{j(m\psi_{q, l+1})}
% % % \end{equation}

% % % With a choice of $\g = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha^{\eta (L -1)} \end{array}}\right]^T$ where we set 
% % % % $\alpha = e^j(\frac{2\pi}{LQ})$
% % % $\alpha = e^j(\frac{\psi_{q}-\psi_{q-1}}{L})$ and suitable $\eta$ (to be determined later), we can write


% % % % \begin{equation}
% % % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{2 \pi(\ell+0.5)}{LQ})}
% % % % \end{equation}

% % % \begin{equation}
% % %     \Tilde{c}_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} g_l e^{jm(\psi_{q-1}+\frac{(\psi_{q}-\psi_{q-1})(\ell+0.5)}{L})}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = \lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l} e^{jm(\psi_{q-1}+\frac{0.5(\psi_{q}-\psi_{q-1})}{L})} 
% % % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})}\lim_{L\longrightarrow \infty} \frac{1}{L}\sum_{l=0}^{L-1} \alpha^{(\eta+m) l}   
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} \alpha^{(\eta + m)Lx}dx
% % % \end{equation}


% % % % \begin{equation}
% % % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\frac{2\pi(\eta + m)L}{LQ}x}dx
% % % % \end{equation}


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \int_{0}^{1} e^{j\xi x}dx
% % % \end{equation}

% % % where $\xi = (\psi_{q}-\psi_{q-1}) (\eta +m )$.


% % % \begin{equation}
% % %     c_q^{(m)} = e^{jm(\psi_{q-1})} \frac{e^{j\xi}-1}{j\xi}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} \frac{e^{j\xi/2}-e^{-j\xi/2}}{j\xi/2}
% % % \end{equation}

% % % \begin{equation}
% % %     c_q^{(m)} = e^{j(m\psi_{q-1} + \frac{\xi}{2})} sinc(\frac{\xi}{2\pi})
% % % \end{equation}

% % % where, $sinc(t) = \frac{sin(\pi t)}{\pi t}$.
















% % % % We first optimize for $\alpha$ by setting the derivative of \eqref{obj_func} to zero, to get: 

% % % % $$\hat{\alpha}=\frac{\sum_{q \in \mathcal{W}_k}\sqrt{\frac{Q}{M_{t}}}(\mathbf{F} \mathbf{v})^{H} \mathbf{D}_{q} \mathbf{g}_q}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}}$$

% % % % Replacing the value of $\alpha$ as above we get to the following optimization problem. 

% % % % \begin{align}
% % % % \left(\mathbf{F}_{\mid \mathbf{g}}, \mathbf{v}_{\mid \mathbf{g}}\right) &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max } \frac{\left|\sum_{q \in \mathcal{W}_k}\sqrt{\frac{2^{\mathbf{B}}}{M_{t}}}\left(\mathbf{D}_{q} \mathbf{g}_q\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}}{\left\|\mathbf{D}^{H} \mathbf{F} \mathbf{v}\right\|_{2}^{2}} \nonumber \\
% % % % &=\underset{\mathbf{F}, \mathbf{v}}{\arg \max }\left|\sum_{q \in \mathcal{W}_k}\left(\mathbf{D}_{q} \mathbf{g}\right)^{H} \mathbf{F} \mathbf{v}\right|^{2}
% % % % \end{align}


% \subsection{UPA Codebook Design Prolem}

% Suppose an $M_h \times M_v$ UPA is placed at the $x-z$ plane, and let $M = M_h M_v$. Let the distance between the antennas that are placed parallel to $z$ axis, be $d_z$, and $d_x$ respectively. One can define,

% \begin{align}
% \mathbf{d}_{M_{a}}\left(\psi_{a}\right) = \left[1, e^{j \psi_{a}} \cdots e^{j\left(M_{a}-1\right) \psi_{a}}\right]^{T} \in \mathbb{C}^{M_{a}}
% \end{align}
% where, $\psi_{h}=\frac{2 \pi d_{x}}{\lambda} \sin \theta \cos \phi \text { and } \psi_{v}=\frac{2 \pi d_{z}}{\lambda} \sin \phi$, and $a$ takes value in the set $\{v, h\}$.  
% The array response vector is then defined as 

% \begin{align}
%     \mathbf{d}_{M}\left(\psi_{v}, \psi_{h}\right) =
%     \mathbf{d}_{M_{v}}\left(\psi_{v}\right) \otimes
%     \mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \in \mathbb{C}^{M}
% \end{align}
% Let $\mathcal{B}_s$ be the angular range under cover. We have, 

% \begin{equation}
%     \mathcal{B}_{s} \doteq \left[-\phi^{\mathrm{B}}, \phi^{\mathrm{B}}\right)
%     \times \left[-\theta^{\mathrm{B}}, \theta^{\mathrm{B}}\right) \label{range_angle}
% \end{equation}

% Notation $\psi^{p,q}_{h}[1:L_h,1 :L_v], \psi^{p,q}_{v}[1:L_v]$

% Let us uniformly divide the angular range  into $Q=Q_{v} Q_{h}$ subregions. For each subregion we have, 

% $$ \mathcal{B}_{p, q} =  \omega_{\phi, p} \times \omega_{\theta, q}$$

% Let $\Delta_{\theta} =  2 \theta^{\mathrm{B}} / Q_{v}$, and $\Delta_\phi =  2 \phi^{\mathrm{B}} / Q_{h}$ be the length of each sub-interval along axis $\theta$, and $\phi$. We have $\omega_{\theta, q} = [\theta_{q-1}, \theta_q)$, and, $\omega_{\phi, p} = [\phi_{p-1},\phi_p)$ where  $\theta_q = -\theta^B + q\Delta_\theta$, and $\phi_p = -\phi^B + p\Delta_\phi$. 


% In the $(\psi_h, \psi_v)$ domain, we can rewrite equation \eqref{range_angle} as, 

% \begin{equation}
%     \mathcal{B}^\psi_{s} \doteq\left[-\psi_h^{\mathrm{B}}, \psi_h^{\mathrm{B}}\right) \times\left[-\psi_v^{\mathrm{B}}, \psi_v^{\mathrm{B}}\right)
% \end{equation}

% and each sub-region similarly can be rewritten in the $\psi$ domain as

% $$ \mathcal{B}^\psi_{ p, q} \doteq \nu_{v}^{p, q} \times \nu_{h}^ {p, q}$$

% % We can then write for each $v_{a, b}$, i.e the $b$-th sub-interval along axis $a$,

% % \begin{equation}
% %     \nu_{v, p} =-\psi_{a}^{\mathrm{B}}+(b-1)\Delta_{a}+\left[0, \Delta_{a}\right)
% % \end{equation}

% Define the reference gain at $(\psi_{h}, \psi_{v}) $ as, 

% \begin{equation}
%     G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) =\left|\left(\mathbf{d}_{M_{v}}\left(\psi_{v}\right)\otimes\mathbf{d}_{M_{h}}\left(\psi_{h}\right)  \right)^{H} \mathbf{c}\right|^{2}
% \end{equation}

% It is straightforward to show that, 

% \begin{equation}
%     \int_{-\pi}^{\pi} \int_{-\pi}^{\pi} G\left(\psi_{v}, \psi_{h}, \mathbf{c}\right) d \psi_{v} d \psi_{h}={(2 \pi)^{2}}
% \end{equation}

% Therefore, for every interval $\mathcal{B}_{ p, q}$ we can derive the ideal gain expression as, 

% \begin{equation}
%     G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)=G_{p,q} \mathds{1}_{\mathcal{B}^\psi_{p, q}}\left(\psi_{v}, \psi_{h}\right)
% \end{equation}

% where $G_{q,p} = \frac{(2\pi)^2}{\delta_{p,q}}$, where $\delta_{p,q}$ is the area of the interval $\mathcal{B}^\psi_{p,q}$. We define the codebook design problem under the UPA structure as follows. 
% % where $G_{q,p} = \frac{(2\pi)^2}{\delta^{p,q}_h\delta^p_v}$, $\delta^p_v = \psi^p_v - \psi^{p-1}_v $, and $\delta^{q, p}_h = \psi^{q,p}_h - \psi^{q-1, p}_h $. Also, let us define $\delta_{q,p} = \delta^{q, p}_h\delta^p_v$. 



% \begin{align}
% & \c^{opt}_{p, q} = \nonumber\\&\underset{\c, \|\c\|=1}{\arg \min } \iint_{\mathcal{B}_{s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \label{init_opt}
% \end{align}

% By partitioning the range of $(\psi_h, \psi_v)$ into the pre-defined intervals, we can rewrite the optimization problem as follows, 

% \begin{align}
% & \c^{opt}_{p, q} = \underset{\c, \|\c\|=1}{\arg \min }\nonumber\\& \sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\iint_{\mathcal{B}^{\psi}_{r,s}}\left|G_{p, q}^{\text {ideal }}\left(\psi_{v}, \psi_{h}\right)-G\left(\psi_{v}, \psi_{h}, \c\right)\right| d \psi_{v} d \psi_{h} \nonumber\\&
%  = \underset{L_h, L_v \rightarrow \infty}{\lim}\sum_{r=1}^{Q_v}\sum_{s=1}^{Q_h}\sum_{l_v =1}^{L_v}\sum_{l_h =1}^{L_h}\frac{\delta^r_v\delta^{r,s,l_v}_h}{L_hL_v}\nonumber\\&
% \left|G_{p, q}^{\text {ideal }}\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_v][l_h]\right)-G\left(\psi^{r,s}_{v}[l_v], \psi^{r,s}_{h}[l_v][l_h], \c\right)\right| \label{alternative_opt}
% \end{align}
% where, 

% \begin{align}
%     &\psi^{r,s}_v[l_v] = \psi^{r-1, s}_v + l_v\frac{\delta_v^r}{L_v}\nonumber\\
%     &\psi^{r,s}_h[l_v][l_h] = \psi^{r, s-1}_h[l_v] + l_h\frac{\delta_h^{r,s, l_v}}{L_h}
% \end{align}

% We can rewrite the optimization problem \eqref{alternative_opt} as, 

% \begin{align}
%     \c_{p,q}^{opt}=\arg \min _{\c, \|\c\|=1} \underset{L_h, L_v \rightarrow \infty}{\lim}\frac{1}{L_hL_v}\left\|\mathbf{G}^{\text {ideal }}_{p,q}-\mathbf{G}(\c)\right\|
% \end{align}


% where, 

% \begin{align}
%     &\mathbf{G}(\c) = \nonumber\\&\left[\delta^1_v\delta^{1,1,1}_hG\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1][1], \c\right) \cdots \right. \nonumber\\ &\left. \delta^{Q_v}_v\delta^{Q_v,Q_h,L_v}_hG\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{v}\right]\left[L_{h}\right], \c\right)\right]^{T} 
% \end{align}

% and, 

% \begin{align}
%     &\mathbf{G}^{\text {ideal }}_{ p, q} = \nonumber\\&\left[\delta^1_v\delta^{1,1,1}_hG^{\text {ideal }}_{ p, q}\left(\psi_{v}^{1,1}[1], \psi_{h}^{1,1}[1][1] \right) \cdots \right. \nonumber\\ &\left. \delta^{Q_v}_v\delta^{Q_v,Q_h,L_v}_hG^{\text {ideal }}_{ p, q}\left(\psi_{v}^{Q_{v}, Q_{h}}\left[L_{v}\right], \psi_{h}^{Q_{v}, Q_{h}}\left[L_{v}\right]\left[L_{h}\right]\right)\right]^{T} 
% \end{align}


% % \begin{align}
% %      &\mathbf{G}^{\text {ideal }}_{ q, p}= \nonumber\\&\left[{\delta_{1,1}} G^{\text {ideal }} _{q, p}\left(\psi^{1}_{h}[1], \psi^{1}_{v}[1], \c\right) \ldots {\delta_{Q_h, Q_v}}G^{\text {ideal }} _{q, p}\left(\psi^{Q_h}_{h}[L_h], \psi^{Q_v}_{v}[L_v], \c\right)\right]^{T} 
% % \end{align}


% Note that we can write, 

% \begin{align}
%     \mathbf{G}^{\text{ideal }}_{p,q} = \frac{{(2\pi)}^2}{\delta_{p,q}} \left(\e_{p,q} \otimes (\boldsymbol{\delta}_{p,q}\odot\mathbf{1}_{L, 1})\right)
% \end{align}

% where, $\boldsymbol\delta_{p,q} = $
% with $\mathbf{e}_{p,q} \in \mathbb{Z}^{Q}$ being the standard basis vector for the $(p,q)$-th axis among $Q$ ones. 








% Now, note that $\mathbf{1}_{L, 1}=\mathbf{g} \odot \mathbf{g}^{*}$ for any equal gain $\mathbf{g} \in \mathbb{C}^L$. Therefore, we can write: 

% % $$\mathcal{G}_{L}=\left\{\mathbf{g} \in \mathbb{C}^{L}:\left(\mathbf{g} \mathbf{g}^{H}\right)_{\ell, \ell}=1,1 \leq \ell \leq L\right\}$$


% \begin{align}
% \mathbf{G}^{\text {ideal }}_{p,q} &=\frac{{2\pi}^2}{\delta_{p,q}}\left(\mathbf{e}_{p,q} \otimes\left((\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\boldsymbol\delta^{(\frac{1}{2})}_{p,q})\odot(\mathbf{g} \odot \mathbf{g}^{*})\right)\right) \nonumber\\
% &=\left(\frac{{2\pi}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\mathbf{g})\right)\right) \nonumber\\&\odot\left(\frac{{(2\pi)}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{p,q}\odot\mathbf{g})\right)\right)^{*} \label{g_id_q_equivalent}
% \end{align}

% Also, note that we can write, 

% % \begin{align}
% %     \mathbf{G}(\c)=\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right) \odot\left(\left(\mathbf{D}_{h}^{H} \otimes \mathbf{D}_{v}^{H}\right) \c\right)^{*}
% % \end{align}
% \begin{align}
%     \mathbf{G}(\c)=\left(\D^H \c\right) \odot\left(\D^H \c\right)^{*}
% \end{align}

% where 

% \begin{align}
%     \D = \left[D^{1,1}_{vh}, \cdots, D^{Q_v,Q_h}_{vh}\right] \in \mathbb{C}^{M_vM_h\times L_vL_hQ_vQ_h}
% \end{align}

% % \begin{align}
% % % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% % &\mathbf{D}_{h, q}(\chi) =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1], \chi \right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right], \chi \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% % &\mathbf{D}_{vh, p,q} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}[1]), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h, q}(\psi_{v}^{p}\left[L_{v}\right]) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% % \end{align}

% \begin{align}
% % &\mathbf{D}_{v} =\left[\mathbf{D}_{v, 1}, \cdots, \mathbf{D}_{v, Q_{v}}\right] \in \mathbb{C}^{M_{v} \times L_{v} Q_{v}} \\
% % &\mathbf{D}_{h} =\left[\mathbf{D}_{h, 1}, \cdots, \mathbf{D}_{h, Q_{h}}\right] \in \mathbb{C}^{M_{h} \times L_{h} Q_{h}} \\
% % &\mathbf{D}_{v, p} =\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p}[1]\right), \cdots, \mathbf{d}_{M_{v}}\left(\psi_{v}^{p}\left[L_{v}\right]\right)\right] \in \mathbb{C}^{M_{v} \times L_{v}}\\
% % &\mathbf{D}_{h, q} =\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{q}[1]\right), \cdots, \mathbf{d}_{M_{h}}\left(\psi_{h}^{q}\left[L_{h}\right]\right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}\\
% \mathbf{D}^{p,q}_{h}(\ell) =&\sqrt{\delta_v^{p}\delta^{p,q,\ell}_h}\left[\mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}[\ell][1] \right), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{h}}\left(\psi_{h}^{p,q}\left[\ell] [L_{h} \right] \right)\right] \in \mathbb{C}^{M_{h} \times L_{h}}, 
% \end{align}

% \begin{align}
%     \mathbf{D}_{vh}^{p,q} =&\left[\mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}[1]\right) \otimes \mathbf{D}_{h}^{p,q}(1), \cdots, \right.\nonumber\\&\left. \mathbf{d}_{M_{v}}\left(\psi_{v}^{p,q}\left[L_{v}\right]\right) \otimes \mathbf{D}_{h}^{p,q}(L_{v}) \right] \in \mathbb{C}^{M_{v}M_{h} \times L_{v}L_{h}}
% \end{align}
% \begin{problem}
% Given an equal-gain vector $\g_{p,q} \in \mathbb{C}^L$, $(p,q) \in \{(1,1), \cdots, (Q_v, Q_h)\}$, find vector $\c_{p,q} \in \mathbb{C}^{M_t}$ such that
% \begin{align}
% &\c_{p,q}=\underset{\c, \|c\|=1}{\arg \min } \lim_{L\rightarrow \infty} \left\|\frac{{2\pi}}{\sqrt{\delta_{p,q}}}\left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})\right)- \D^H \c\right\|^{2} \label{obj_func}
% \end{align}
% \label{main_problem_UPA}
% \end{problem}


% Note that the solution to problem \ref{main_problem_UPA} is the limit of the sequence of solutions to a least-square optimization problem as $L$ goes to infinity. For each $L$ we find that,
%  \begin{align}
%  {\c}^{(L)}_{p,q} &= {\frac{{2\pi}}{\sqrt{\delta_{p,q}}}}(\D \D^H)^{-1} \D  \left(\mathbf{e}_{p,q} \otimes (\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})\right) \nonumber\\& =\sigma \D^{p,q}(\boldsymbol\delta^{(\frac{1}{2})}_{L,1}\odot\mathbf{g}_{p,q})
% \end{align}
% where $\sigma = \frac{2\pi \sqrt{\delta_{p,q}}}{L\sum_{(q,p)= (1,1)}^{(Q_h, Q_v)} \delta_{p,q}}$, noting that it holds that, 

% Noting that it holds that, 

% \begin{align}
%     (\D\D^H) = \left(L\sum_{(p,q)= (1,1)}^{(Q_h, Q_v)}\sum_{(l_v,l_h)= (1,1)}^{(L_h, L_v)} \delta_{v}^p\delta^{p,q,l_v}_{h}\right)\I_{M_t}
% \end{align}

% \begin{problem}
% Find equal-gain $\g_{p,q} \in \mathbb{C}^L$, $(q,p) = (1,1), \ldots, (Q_h, Q_v)$, such that
% \begin{equation}
%  \g_{q,p} = \underset{\g}{\arg\min }\left\| abs(\D^H \c_{q,p})- {2\pi} abs(\mathbf{e}_{q,p} \otimes \mathbf{g})\right\|^{2} \label{g_final_eq}
% \end{equation} 
% where $abs(.)$ denotes the element-wise absolute value of a vector.
% \label{g_problem}
% \end{problem}


% \begin{proposition}
% The minimizer of \eqref{g_simple_final_eq} is in the form $\g_q = \left[{\begin{array}{cccc} 1& \alpha^\eta &\cdots & \alpha_h^{\eta (L_h -1)}\alpha_v^{\eta (L_v -1)} \end{array}}\right]^T$ for some $\eta$ where $\alpha_h = e^{j(\frac{\delta^{q,p}_h}{L_h})}$ and $\alpha_v = e^{j(\frac{\delta^p_v}{L_v})}$. \label{proposiiton_g}
% \end{proposition}

%  \begin{align}
%      {\c_{p,q}}^{(L)} & = \sigma \sum_{(l_v, l_h)=(1,1)}^{(L_v, L_h)}g_{p,q, l}\mathbf{d}_{M_t}\left(\psi^{p,q}_{v}[l_v], \psi^{p,q}_{h}[l_v][l_h]\right)  \nonumber\\
%      & = \sigma \sum_{l=1}^L g_{q,p,l}\left[{\begin{array}{ccc}
%      1 &\cdots & e^{j\left( (M_v-1)\psi^{p,q}_{v}[l_v] + (M_h-1)\psi^{p,q}_{h}[l_v][l_h]\right)}\\
%      \end{array}}\right]^T   
%     %  \nonumber\\& = \left[{\begin{array}{ccc}
%     %  \sigma\sum_{l=1}^L g_{q, p, l}& \cdots & \sigma\sum_{l=1}^L g_{q,p, l}e^{j\left((M_h-1)\psi^q_{h}[l] + (M_v-1)\psi^p_{v}[l]\right)}\\
%     %  \end{array}}\right]^T
% \end{align}

% We can then write 

% \begin{align}
%     c_{p,q, m_v, m_h} &= \lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} \nonumber \\&\delta^p_v\delta_h^{p,q,l_v}g_{p,q, l_v, l_h}e^{j\left(m_v\psi^{p,q}_{v}[l_v]+ m_h\psi^{p,q}_{h}[l_v][l_h] \right)}
% \end{align}


% \begin{align}
%     c_{p,q, m_v, m_h} &=  \nonumber\\&\lim_{L_h, L_v\rightarrow \infty} \frac{1}{L_hL_v}\sum_{(l_h, l_v)=(1,1)}^{(L_h, L_v)} \delta^p_v\delta_h^{p,q,l_v}g_{p,q, l_v, l_h}\nonumber \\&e^{j\left(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v})+ m_h(\psi^{p,q-1}_{h}[l_v] + l_h\frac{\delta^{p,q,l_v}_h}{L_h}) \right)}
% \end{align}


% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} S^{(l_v)}
% \end{align}

% where, 

% \begin{align}
%     S^{(l_v)} &= \lim_{ L_h\rightarrow \infty}\frac{\delta^{p,q,l_v}_h}{L_h}\sum_{l_h=1}^{L_h}e^{j(m_h(\psi^{p,q-1}_{h}[l_v] + l_h\frac{\delta^{p,q,l_v}_h}{L_h}) + y\gamma \frac{l_h}{L_h})} \nonumber\\& = \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi})
% \end{align}

% with $\xi = {\delta^{p,q,l_v}_h}{m} + y\gamma$. Therefore, it. holds that, 

% \begin{align}
%     c_{p,q, m_v, m_h} &=  \lim_{ L_v\rightarrow \infty} \frac{\delta^p_v}{L_v}\sum_{l_v=1}^{L_v} e^{j(m_v(\psi^{p-1,q}_{v}+l_v\frac{\delta^p_v}{L_v}) + x\eta\frac{l_v}{L_v})} \delta^{p,q,l_v}_h e^{jm_h\psi^{p,q-1}_{h}[l_v]}sinc(\frac{\xi}{2\pi})
% \end{align}

==> cramer-rao.tex <==

\subsection{Derivation of Cramer-Rao Bound}

In this section, we derive the Cramer-Rao lower bound on the MSE estimate of any non-biased CFO estimator which is based on the observation of $r^{(m)}(i)$ for all $m$, $1 \leq m \leq M$ and available time index $i$. %\subsection{Deriving the Bound} 
First, we note that the channel taps are samples of zero mean circularly symmetric complex Gaussian distributions. Hence, over the ensemble of the channel realizations, $r^{(m)}[i]$ will also follow zero-mean circularly symmetric complex Gaussian distributions. In order to find the joint distribution of $r^{(m)}[i]$, for all available $i$ and $m$, it suffices to find the covariance matrix. % of $r^{(m)}(i)$ is given by $\eta^{(m)} + \sigma_z^2$. 
Let $X$ be defined as a vector containing all $r^{(m)}[i]$, for $K$ OFDM symbols, $M$ antennas and $2L$ values of $i$, i.e.,  $i = 1, 2, \ldots, L, N+1, N+2, \ldots, N+L$. We have
\begin{align}
    \x = [ r^{(1)}[1], \ldots, r^{(1)}[K\tilde{N}], r^{(2)}[1], \ldots, r^{(M)}[K\tilde{N}]]^T 
\end{align}
The entries of the covariance matrix $\mathbb{E}\{X X^*\}$ is given as follows. If $m_1 \neq m_2$ and $i_1 \neq i_2$, $j \neq 0 $ and $j \neq N$, we have
\begin{align}\label{eq:mean_u}
    \mathbb{E}\{r^{(m)}[k \tilde{N} +i](r^{(m)}[k \tilde{N} +i])^*\} = \eta^{(m)} + \sigma_z^2, \\    
    \mathbb{E}\{r^{(m)}[k \tilde{N} +i](r^{(m)}[k \tilde{N} +N+i])^*\} = \eta^{(m)}_i e^{j 2 \pi \theta} \\
    \mathbb{E}\{r^{(m)}[k \tilde{N} +i](r^{(m)}[k \tilde{N} +i+j])^*\} = 0, \\
    \mathbb{E} \{r^{(m_1)}[k \tilde{N} +i](r^{(m_2)}[k \tilde{N} +i])^*\} = 0 \\
    \mathbb{E} \{r^{(m_1)}[k \tilde{N} +i_1](r^{(m_2)}[k \tilde{N} +i_2])^*\} = 0
\end{align}
Let us define the vector $\v^{(m)}_{k,i} = [r^{(m)}[k \tilde{N}+i], r^{(m)}[k \tilde{N}+N+i]]^T$, and let $\R^{(m)}_i$ be the covariance matrix of $\v^{(m)}_{k,i}$. The distribution of $\x$ is given by
\begin{align} 
    f_X(\x, \theta) &= 
    \prod_{m, 1 \leq m \leq M} \nonumber \\&\left( \prod_{i, 0 \leq i \leq 2L} \frac{1}{\pi^2 \left| \R^{(m)}_i \right|} \exp \left( -\v^{(m)^*}_{k,i} \R^{(m)}_i \v^{(m)}_{k,i} \right) \right)^K 
\end{align}
The Cramer-Rao bound can be found by calculating the Fisher information content of the log-likelihood function defined as
\begin{align}
    I(\theta) &= - \mathbb{E} \left\{ \frac{\partial^2 \log(f_X(\x, \theta))}{\partial \theta^2}\right\} \\
    &= - \mathbb{E} \left\{  \sum_{m, 1 \leq m \leq M} \sum_{i, 0 \leq i \leq 2L} \frac{4K \pi^2}{\left| \R^{(m)}_i \right|} \v^{(m)^*}_{k,i} \Q^{(m)}_i \v^{(m)}_{k,i}  \right\} 
\end{align}
where
\begin{align}
    \Q = \left[ \begin{tabular}{cc}
     0 & $-\eta^{(m)}_i e^{j 2 \pi \theta}$ \\ $-\eta^{(m)}_i e^{j 2 \pi \theta}$ & 0 \end{tabular} \right]
\end{align}

Hence, we have
\begin{align}
    I(\theta) = 8K \pi^2 \sum_{m, 1 \leq m \leq M} \sum_{i, 0 \leq i \leq 2L} \frac{ \eta^{(m)^2}_i}{( \eta^{(m)} 
    + \sigma_z^2)^2 - \eta^{(m)^2}_i}
\end{align}

The Cramer-Rao bound is then given by the inverse of the fisher information $I(\theta)$.

% % \section{Alternative Fine Estimation Based on the Theoretical MSE Bound}


% % In this section, we first derive the theoretical MSE bound. Then, we provide an alternative algorithm for the adaptation of the value of $\Lambda$ in order to boost the accuracy of the proposed CFO estimation based on the derived theoretical MSE bound. 

% % \subsection{Derivation of the MSE Bound}

% % Consider the estimator of the form 
% % \begin{align} \label{eq:zeta}
% %     &\xi = \frac{1}{2 \pi} \angle \frac{1}{KM} \sum_{k=1}^{K} \sum_{m=1}^{M}  \sum_{l=S} r^{(m)}[k\tilde{N}+l] 
% %     r^{(m)}[k\tilde{N}+N+l]^* \nonumber \\
% %     &\:\: = \frac{1}{2 \pi} \angle \frac{1}{KM}  \sum_{k=1}^{K} \sum_{m=1}^{M}  \sum_{l=S} u_{k,m}[l]
% %     \nonumber \\
% %     &\:\: = \frac{1}{2 \pi} \angle  U
% % \end{align}
% % where $S \subset \{0, 1, \ldots, 2L-1\}$.  We note that the mean of $U$ is given by
% % \begin{align}
% %     \mathbb{E}\{U\} = \sum_{m=1}^{M} \sum_{l=S} \eta^{(m)}_l e^{j 2 \pi \theta}
% % \end{align}
% % Hence, we can write
% % \begin{align}
% %     U = \mathbb{E}\{U\} + \delta
% % \end{align}
% % where $\mathbb{E}\{\delta\} = 0$. On the other hand 
% % \begin{align}\label{eq:UUP}
% %     \mathbb{E}\{U U^* \}  = \mathbb{E}\{U\} \mathbb{E}\{U\}^* + \mathbb{E}\{\delta \delta^* \}
% % \end{align}
% % In order to compute $\mathbb{E}\{U U^* \}$, we use the fact that  $u_{k_1,m_1}[l_1]$ and $u_{k_2,m_2}[l_2]$ are uncorrelated if either of $k_1,m_1$ or, $l_1$  are not equal to $k_2,m_2$, or $l_2$, respectively. Hence, it suffices to compute the individual terms of the form $\mathbb{E}\{u_{k,m}[l] u_{k,m}[l]^* \}$. 
% % \begin{align}
% %     &\mathbb{E}\{u_{k,m}[l] u_{k,m}[l]^* \} = 
% %     \mathbb{E}\{r^{(m)}[k\tilde{N}+l] \nonumber \\
% %     &r^{(m)}[k\tilde{N}+N+l]^* r^{(m)}[k\tilde{N}+l]^* 
% %     r^{(m)}[k\tilde{N}+N+l] \}
% % \end{align}
% % In the above expressions, each term $r^{(m)}[.]$ is comprised of the summations of the terms in the form of $\theta[i-l] x[i-l] h^{(m)}_l$ plus a noise $z^{(m)}[i]$. We note that $x[i]$ and $x[j]$ for $i \neq j$ are independent and also $h^{(m_1)}_l$ and $h^{(m_2)}_k$ are independent if either $m_1 \neq m_2$ or $l \neq k$. The terms in $u_{k,m}[l] u_{k,m}[l]^*$ with respect to the components of the input vectors $x[.]$ are in the form $x[i_1]x[i_2]^* x[i_3]x[i_4]^*$, except for the all noise term, and the expectation over $x$'s are nonzero only and only if the terms are in one of the following forms $x[i]x[i]^*$, $x[i]x[i]^* x[i]x[i]^*$ or $x[i]x[i]^* x[j]x[j]^*$, for $j \neq i$.
% % We have
% % \begin{align}
% %     &\mathbb{E}\{u_{k,m}[l] u_{k,m}[l]^* \} = \sigma_x^4 \sum_{i=0}^{l} \mathbb{E}\{ |h^{(m)}_i|^4 \} \nonumber \\
% %     &+ 2 \sigma_x^4 \sum_{i=0}^{L-1} \sum_{j=0}^{L-1} \mathbb{E}\{|h^{(m)}_i|^2 |h^{(m)}_j|^2\} \nonumber \\
% %     &+ 2 \sigma_z^2 \sigma_x^2 \sum_{i=0}^{L-1}  \mathbb{E}\{|h^{(m)}_l|^2\} + \sigma_z^4  \nonumber \\
% %     &= \mathbb{E} \{( \sum_{i=0}^{L-1} |h^{(m)}_i|^2 |x[l-i]|^2 + \sigma_z^2) (\sigma_x^2 \sum_{l=0}^{L-1} |h^{(m)}_l|^2 + \sigma_z^2) \} \nonumber \\
% %     &= (\sigma_x^2 \sum_{l=0}^{L-1} |h^{(m)}_l|^2 + \sigma_z^2)^2 + (\sigma_x^2 \sum_{i=0}^{l} |h^{(m)}_i|^2)^2 \nonumber \\
% %     &= (\eta^{(m)} + \sigma_z^2)^2 + \eta^{(m)^2}_l
% % \end{align}
% % jksdjkg




==> proposed.tex <==
\section{Proposed Beam Alignment Scheme}
\label{sec:proposed}


==> related_work.tex <==
\section{Related Work}
\label{sec:relatedwork}
 

==> tradeoff.tex <==
\section{Main Results}\label{sec:main_results}
\label{sec:results}


==> tulip_proof.tex <==
\section{Problem Formulation}
\label{sec:problem}

\begin{defn}
A contiguous beam, say scanning beam, is denoted by its angular coverage interval (ACI). For example a beam $i$ is denoted as $[s_i,e_i)$ where $s_i$ is the starting point (angle) and $e_i$ is the ending point (angle). 
\label{defn: contiguous}
\end{defn}



\begin{defn}
A direction is defined on the azimuth angles, say, counter-clockwise. The ACI as well as the starting and the ending point of a beam is measured with respect to this direction. For example, one may have a beam starting at $3\pi/2$ and ending at $\pi/2$ which is represented as $[ 3 \pi /2, \pi/2)$.
\label{defn: loop}
\end{defn}

\begin{defn}
Consider a set of points $a_1, a_2, \ldots, a_n$, $n\geq3$ on a circle. For any three indices $1 \leq i, j, k \leq n$, we write $a_i \prec a_j \prec a_k$ (and read as  $a_i$ precedes $a_j$ precedes $a_k$) if by starting from point $a_i$ and moving in the defined direction (say counter clockwise) we first encounter $a_j$ and then encounter $a_k$ before reaching $a_i$ again. Equivalently, we write $a_k \succ a_j \succ a_i$ and read $a_k$ succeeds $a_j$ succeeds $a_i$. Please note that the precedence relation requires at least three points to be specified.
\label{defn: prec_succ}
\end{defn}


\begin{defn}
Consider $b$ beams and denote them by beam $i$, $i \in B$ where $B = {1, 2, \ldots, b}$ denotes the set of all possible beam. For a given subset $C \subset B$, we define a component beam $\omega_C$ as a beam (possibly comprised of an interval or a collection of intervals) where each differential arc of the beam contains all the beams in $C$ and does not contain any beam which is not in $C$. The set $C$ is called the \emph{spawning set} of $\omega_C$ and its cardinality is called the \emph{degree} of $\omega_C$. A component beam may also be represented by its spawning set $C$.  We say a \emph{component beam has a beam $i$ in its intersection} if the beam $i$ belongs to its spawning set.
\label{defn:component}
\end{defn}

% \begin{defn}
% A component beam is always a subset of an intersection of scanning beams. The minimal number of beams for which the component beam is a subset of intersection of those beams is called the \emph{spawning set} and its cardinality is called the \emph{degree} of that component beam. We say a \emph{component beam has a beam $i$ in its intersection} if the beam $i$ belongs to its spawning set.
% \label{defn:degree}
% \end{defn}

\begin{defn}
Consider a set of scanning beam as $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that without loss of generality $s_1 \prec s_2 \prec \ldots \prec s_b$. For any $i$ and $j$, if $s_i \prec s_j \prec e_j \prec e_i$ then we say beam $j$ is nested in beam $i$ and beam $i$ is the host of beam $j$. If beam $j$, $j>i$ is nested in beam $i$ and there is no other beam $k$, $j > k > i$ that is nested in $i$, we say the beam $j$ is the first nested beam in beam $i$.  
\label{defn:nested}
\end{defn}

\begin{defn}
We define the following operators and notations on spawning set. Let spawning set be denoted by $C, D, E, F, X, Y$, etc., and the set of spawning sets be represented by $\mathcal{C}, \mathcal{E}$, etc., e.g., $\mathcal{C} = \{C, D\}$, and $\mathcal{E} = \{E, F\}$. The union of two spawning set $C \cup D$ is denoted by $CD$. The product of two sets of spawning sets $\mathcal{C}$ and $\mathcal{E}$ is denoted by $\mathcal{C} \times \mathcal{E}$ and is defined as a set that contains the union of any pair of sets such that one set belongs to the first and the other one belongs to the second set of spawning sets, i.e., $\mathcal{C} \times \mathcal{E} = \{X, X = X_1 X_2, X_1 \in \mathcal{C}, X_2 \in \mathcal{D}\}$. For example $\{C,D\} \times \{E,F\} = \{CE, CF, DE, DF\}$. The multiplication of the set of spawning sets $\mathcal{C}$ by itself may be represented as $\mathcal{C}^2 = \mathcal{C} \times \mathcal{C}$. The higher power $k > 2$ may be defined recursively as $\mathcal{C}^k = \mathcal{C}^{k-1} \times \mathcal{C}$.
\label{defn:product}
\end{defn}

\begin{defn}
For a set of spawning sets $\mathcal{C}$ and an spawning set $D$ the \emph{back division} operator is defined as $\mathcal{C} \setminus D= \{X, DX \in \{D\} \times \mathcal{C}, D \cap X = \emptyset \}$.
\label{defn:back-division}
\end{defn}

If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $\setminus$ has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$

\begin{defn}
For a set of spawning sets $\mathcal{C}$ and an spawning set $D$ the \emph{forward division} operator is defined as $\mathcal{C} / D= \{X, DX \in \mathcal{C} \}$.
\label{defn:forward-division}
\end{defn}

\begin{defn}
For a set of spawning sets $\mathcal{C}$ and two spawning set $D$, $E$ the \emph{forward division} operator is defined as
$$\mathcal{C} / \{D,E\}= \{X, ((D-A)X \in \mathcal{C} \setminus E \wedge (E-A)X \in \mathcal{C} \setminus D) \lor$$
$$ (DEX \in \mathcal{C}), A = D \cap E  \}$$.
$$\mathcal{C} / \{D,E\}= \{X, (DX \in \mathcal{C} \setminus E \wedge EX \in \mathcal{C} \setminus D) \lor (DEX \in \mathcal{C} \setminus A)\}$$.
$$\mathcal{C} / \{D,E\}= \{X, (DX \in \mathcal{C} \setminus A \wedge EX \in \mathcal{C} \setminus A) \lor (DEX \in \mathcal{C} \setminus A), A = D \cap E \}$$.
\label{defn:forward-division2}
\end{defn}

If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $/$ had precedence on $\setminus$ which in turn has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$

\begin{properties}
For a set of spawning sets $\mathcal{C}$ and a spawning sets $A$, $D$, $E$, $E \cap A \emptyset$, we have
\begin{align}
    \mathcal{C} \setminus AD = (\mathcal{C} \setminus A) \setminus D \\
%    |A \times \mathcal{C}| = |A \times \mathcal{C} \setminus A| \\    
    A \times \mathcal{C} = A \times \mathcal{C} \setminus A \\
    (A \times \mathcal{C}) \cap (AD \times \mathcal{C}) = A \times (\mathcal{C} - \mathcal{C} \setminus D) \\
    |(A \times \mathcal{C}) \cap (AD \times \mathcal{C})| \leq |\mathcal{C} - \mathcal{C} \setminus D| \\
    |AD \times \mathcal{C}| \leq |A \times \mathcal{C}| \\
    |A \times \mathcal{C}| = |\mathcal{C} \setminus A| \\
%    |\{A,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus E| - |(\mathcal{C} / A) \cap (\mathcal{C} / E) | \\
    |\{A,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus E| - |\mathcal{C} / \{D, E\}| \\
%    |\{A,AE\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus AE| - |(\mathcal{C} / AE) \cap (\mathcal{C} / E) | \\
    |\{A,D,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus D| + |\mathcal{C} \setminus E| \nonumber \\
    - |\mathcal{C} / \{A, D\}| - |\mathcal{C} / \{A, E\}| - |\mathcal{C} / \{D, E\}| \nonumber \\
    + |(\mathcal{C} / \{A, D\}) \cap (\mathcal{C} / \{A, E\}) \cap (\mathcal{C} / \{D, E\})| \\
     |\{A_i\}_{i \in [n]} \times \mathcal{C}| = \sum_{i=1}^n |\mathcal{C} \setminus A_i|  \nonumber \\
    - \sum_{s_2 \in S_2[n]} T(s_2) + \sum_{s_3 \in S_3[n]} |\cap_{s_2 \in s_3} T(s_2)| \nonumber \\
    - \sum_{s_4 \in S_4[n]} |\cap_{s_2 \in s_4} T(s_2)| + \ldots \\ 
    \mbox{where } S_k[n] = \{ \{i_1, \ldots, i_k\},  i_l \in [n] \nonumber \\
    \mbox{for } 1 \leq l \leq k, i_1 < i_2 < \ldots < i_k \} \nonumber \\
    \mbox{and } T(s_2) = \mathcal{C} / \{A_{i_1}, A_{i_2}\}, \mbox{for } s_2 = \{i_1, i_2\} \nonumber
\end{align}
\label{defn:division-properties}
\end{properties}

The property 3 may be valid for the spawning sets of a single beam only and the extension may be different. I have to think about it more. The property 4 is derived from property 3.

\begin{defn}
A set of scanning beam has Tulip design if there exist an ordering of the beam in the form of $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that $e_{i-1}, s_{i+1} \in (s_i,e_i)$.   
\label{defn:tulip}
\end{defn}

\begin{defn}
If a set of beams $B' \subset B, B = \{1, 2, \ldots, b\}$, is used for probing, the feedback sequence is a ternary sequence of length $b$ where the position $i$ corresponds to the feedback of beam $i$ and it is set to $1$, $0$ for positive and negative feedback, respectively. If the beam $i$ is not used for probing the position $i$ in feedback sequence is set to $x$. Corresponding to a feedback sequence, we define a \emph{feedback index set (FIS)} which contains the indices of the beams for which a positive feedback is received. The cardinality of th index sequence is defined as the degree of the feedback sequence.
\label{defn:FBS}
\end{defn}

\begin{defn}
A set of scanning beam has Tulip design if there exist an ordering of the beam in the form of $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that $e_{i-1}, s_{i+1} \in (s_i,e_i)$.   
\label{defn:tulip}
\end{defn}

\begin{lemma}
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 1$ path.
\label{lemma:Tulip_1}
\end{lemma}

\proof
The proof relies on the fact that $b$ contiguous beams have total of $2b$ starting and ending points and hence can generate at most $2b$ component beams. On the other hand for $p=1$ a feedback sequence is valid only and only if the set of the indices of the beam with positive feedback corresponds to an spawning set of a component beam that is realized by the set of scanning beams. Since there are at most $2b$ component beam, there is only $2b$ possible feedback sequences and Tulip design already provides $2b$ component beams. We note that the Tulip structure is not the only optimal design for $p=1$.

\begin{lemma}
For a channel with $p=2$ paths, a set of scanning beams with Tulip design generates $1, 3, 7$, and  $15$ feedback sequences for $b = 1, 2, 3$, and 4 beams, respectively, and generates $2b(b-2)$ feedback sequences for $b > 4$ beams. 
\label{lemma:Tulip_2_count}
\end{lemma}

\proof
The proof is simply follows from a direct counting argument.
There are $b$ component beams of degree 1 with spawning sets $\{1\}, \{2\}, \ldots, \{b\}$ that are directly part of the Tulip design. For $b>1$, there are $b \choose 2$ feedback sequences of degree 2 corresponding to the beam index sets $\{12\}, \{13\}, \ldots, \{1b\}, \{23\}, \{24\}, \ldots, \{2b\}, \ldots, \{(b-1)b\}$. A degree 2 feedback sequence corresponding to an index set $\{ij\}$ can be generated by selecting path 1 and path 2 inside the component beams $\{i\}$ and $\{j\}$, respectively. For $b > 2$, a feedback sequence of degree 3 may be generated by selecting a path in a component beam of degree 2 and a path in a component beam of degree $1$. In the following consider the indices of the beam in mod $b$. In other words, the beam $b+1$ is the same as beam $1$. There are total of $b(b-3)$ feedback sequences of type $i(i+1)k$. Consider the set $C_i = \{ i(i+1)k, k \neq i, k \neq (i+1)\}$. There are $b$ sets $C_i, i = 1, 2, \ldots, b$, and each set $C_i$ has $b-2$ distinct feedback sequences and there are exactly $b$ feedback sequences of the form $i(i+1)(i+2)$ which appear in all sets 
$C_i, i = 1, 2, \ldots, b$ exactly twice. Hence the union $\cup_{i \on B} C_i$ contains exactly $b(b-3)$ distinct feedback sequences. Similarly, for $b>4$, it can be argued that there are exactly $b(b-3)/2$ degree 4 feedback sequences of type $i(i+1)j(j+1)$, $i+1 \succ j$, $j+1 \succ i$ that are generated by having one path in the component beam $i(i+1)$ and another in the component beam $j(j+1)$. For $b=4$, there is only one feedback sequence $1234$ that is generated by having one path in component beam $12$ and one path in component beam $34$. Summing all the feedback sequences of degree 1 to degree 4 proves the statement of the lemma.

\begin{lemma} [NOT REQUIRED]
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 2$ path, for an arbitrary distribution of channel AoD that is nonzero on $[0, 2 \pi)$
\label{lemma:Tulip_2}
\end{lemma}

\proof
Lemma~\ref{lemma:Tulip_1} proves the optimality of Tulip design for a channel with single path, i.e., $p=1$. Lemma~\ref{lemma:Tulip_2}, extends this optimality to the case of $p=2$, however, the proof is considerably more involved. 

Here, we first provide the sketch of the proof and then formally get into the details. Lemma~\ref{lemma:Tulip_2_count}, counts the number of feedback sequences that is generated by Tulip design. It is relatively easy to check for small numbers of $b \leq 5$ that no other set of scanning beams can generate more number of feedback sequences as Tulip design. For the case of $b>5$, we use induction to prove the lemma. For each step of the induction for $b+1$ beams, we select a beam and remove it. The resulting structure cannot generate more than $2b(b-2)$ feedback sequences per induction assumption. We show that adding the $b+1$ beam back to the previous structure cannot add more than $4b-2$ new feedback sequences. Hence, any structure with $b+1$ beams can generate at most $2b(b-2) + (4b - 2) = 2(b^2-2b+2b-1) = 2(b+1)(b-1) = 2(b+1)((b+1)-2)$ which is already achievable with Tulip structure. 

To prove the induction step for $b+1$ beams, we assume that we have an structure that is generating the maximum number of feedback sequences. First, we note that we can assume that the set of points $P$ consisting the starting points and ending points of each beam has exactly $2b$ points. Otherwise, if two points coincides, one can generate a new sets of beams by slightly moving one of the points. For such new beams the number of feedback sequences would not be less. Second, we prove that there is no beam that is nested in all other beams. In other words, if there is a beam where its starting point and ending point are immediately succeeding in the loop that consists of all the point of $P$ and there is no other points in $P$ that lie in between the staring an ending point of this beam. Suppose not, then by removing this beam the resulting number of feedback sequences is not more than $2b(b-2)$. By adding this $b+1$ beam back to the structure, one cannot generate more than $2b$ new feedback sequences, hence it is resulting less than $2(b+1)((b+1)-2)$ feedback sequences and it contradict the assumption that this structure generates the maximum number of feedback sequences.

Third, consider the case that the starting and the ending point of the beam $b+1$ is within two different component beams of the first $b$ beams. Let $C_b$, and $C_{b+1}$ denotes the set of component beams for the first $b$ beam and all $b+1$ beams, respectively. Assume the component beams in $C_b$ are denoted by $A_i$, i.e., $C_b = \{ A_1, A_2, \ldots, A_{2b}\}$. Hence, without loss of generality, there exist some $i$ and $j$ such that $C_{b+1} = (C_b - \{A_{i+1}, \ldots, A_(j-1)\}) \cup \{ (b+1)A_i, (b+1)A_{i+1}, \ldots, (b+1)A_j\}$, where $i$ and $j$ are the indices of the component beams where the starting and ending points of the beam $b+1$ fall within them.

The sets of FIS $F_b$ and $F_{b+1}$ for the first $b$ beams and all $b+1$ beams and $p=2$ is obtained as $F_b = C_b \times C_b$ and $F_{b+1} = C_{b+1} \times C_{b+1}$, respectively. We have
\begin{align}
    F_{b+1} &= \{A_k A_l\}_{k \in S, l \in S} \cup \{(b+1) A_k A_l\}_{k \in T, l \in T} \\
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in T} \\  
    &= \{A_k A_l\}_{k \in S, l \in S} \\
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in V} \\ 
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in U} \\
    &\cup \{(b+1) A_k A_l\}_{k \in U, l \in V} \\
    &\cup \{(b+1) A_k A_l\}_{k \in U, l \in U} 
    ,\mbox{and}\\
    F_{b} &= \{A_k A_l\}_{k \in B, l \in B} \\
    &= \{A_k A_l\}_{k \in S, l \in S} \\ 
    &\cup \{A_k A_l\}_{k \in S, l \in U} \\
    &\cup \{(A_k A_l\}_{k \in U, l \in U} 
\end{align}
where $S = \{1, 2, \ldots, i\} \cup \{j, j+1, b\}$ and $T = \{i, i+1, \ldots, j\}$, $U = \{i+1, i+2 \ldots, j-1\}$, $V = \{i, j\}$. I did not write the rest of the proof.

\begin{lemma}[NOT REQUIRED]
We say that there is a loop in the set of scanning beams, if there exist two beams $i$ and $j$ denoted by $[s_i,e_i)$ and $[s_j,e_j)$, respectively, such that $s_j \prec e_i \prec s_i \prec e_j$. If there is a loop in the set of scanning beams, it is always possible to open the loop by exchanging the beams $i$ and $j$ with two new beams that are not forming a loop such that as a result of opening the loop the number of feedback sequences is not decreased. 
\label{lemma: loop-free}
\end{lemma}

\proof
Define the following for intervals: $A = [s_j, e_i)$, $B = [e_i, s_i)$, $C = [s_i, e_j)$, $D = [e_j, s_i)$. WLOG, assume $i = 1$ and $j = 2$. Obviously, each component beam belong to at least one of these four sets. A component beam that belongs to set $A$ or $C$ has at least beam 1 and 2 in its intersection. Consider the component beam $\omega_{12}$. There are four cases: (i) $\omega_{12} \subset A$ and $\omega_{12} \subset C$, (ii) $\omega_{12} \not \subset A$ and $\omega_{12} \not \subset C$, (iii) $\omega_{12} \not \subset A$ and $\omega_{12} \subset C$, (iv) $\omega_{12} \subset A$ and $\omega_{12} \not \subset C$. For the case (i) to (iii) we set $E = A$ and for the case (iv) we set $E = C$. By removing the interval $E$ from both beams we generate two new beams with ACIs $[s_i,e_i)-E$ and $[s_j,e_j)-E$ that are not forming a loop. It remains to verify that the number of possible feedback sequences for the new beam set is not decreased. Since the old and new beam set only differ in interval $E$, any feedback sequence (FS) that is generated without a path in $E$ using old beam set can be generated by the new beam set as well. Now consider the case that there is still one path in $E$. Let $F$ denote the indices of the beams for a feedback sequence generated by a given set of paths including one path in $E$. For the old beam set, we always have $\{1,2\} \subset F$ and we can define $F' = F - \{1,2\}$. For the new set depending on where the paths outside $E$ are the indices of the beams for the feedback sequence for the new set is given by either $F'$, $F' \cup \{1\}$, $F' \cup \{2\}$, or $F' \cup \{1,2\}$ which are all different.


\begin{lemma}[NOT REQUIRED]
For a set of scanning beam $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ where $s_1 \prec s_2 \prec \ldots \prec s_b$, if the beam $j$ is the first nested beam in beam $i$, then exchanging the beam $i$ and $j$ with the two new beams $[s_i,e_j)$ and $[s_j, e_i)$, the number of possible feedback sequences is not decreased. 
\label{lemma: nested}
\end{lemma}

\proof


\begin{lemma}[NOT REQUIRED]
There exists an algorithm which can remove all possible nested beams to generate an un-nested set of scanning beams such that for the resulting scanning beams the number of possible feedback sequences is not decreased.
\label{lemma: termination}
\end{lemma}

\proof 
Define the ACIs of the set of scanning beams as $A_1, A_2, \ldots, A_b$ where $A_i = [s_i, e_i)$ and $s_1 \prec s_2 \prec \ldots \prec s_b$.
Consider the following algorithm. For $k = 1:b$, For $l = 1:k-1$, If $A_k$ is nested in $A_l$, exchange $e_k$ and $e_l$, endif, endfor, endfor. It can be easily verified that at the end of this algorithm, there is no nested beam. On the other hand, since each step of the algorithm uses the exchange of the end points of a nested beam with its parent (define parent of the nested beam), hence, using lemma~\ref{}, the number of possible feedback sequence is not decreased in each step and hence it is not decreased overall.

\proof
Consider any ordered


\begin{lemma}[NOT REQUIRED]
For an un-nested set of scanning beams, if there exists a component beam of degree three or more, there exist a new set of scanning beams with reduced degree for the same component beam for which the number of possible feedback sequences is not decreased.
\label{lemma:un-nested}
\end{lemma}

\begin{thm}
The most distinguishable set, i.e., the set with the largest possible size, may be obtained through Tulip design defined by a set of single span SBs $\mathcal{B}=\left\{\Phi_{i}\right\}, i \in[b]$, where each beam may only have intersection with its adjacent beams with the exception of $\Phi_{1}$ and $\Phi_{b}$ for which the intersection might be nonempty. This means $\Phi_{i} \cap \Phi_{j}=\varnothing, 1<$ $|i-j|<b$
\end{thm}

% \proof
% Lemma~\ref{lemma:Tulip_1} proves the statement of the theorem for the case of the channel with $p=1$ path. Here, we provide the proof for the case of $p>1$. We note that the set FIS $\mathcal{F}$ for the channel with $p$ path is obtained as $F = \mathcal{C}^p$ where $\mathcal{C}$ is the set of spawning set of all component beams.  

% Consider a set of scanning beams and select an arbitrary scanning beam and name it beam 1. Then select the other beams such that for the set of scanning beams $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ we have $s_1 \prec s_2 \prec \ldots \prec s_b$. 

% One of the following cases may occur.
% \begin{itemize}
%     \item We have $s_1 \prec e_1 \prec s_2$. In this case the arc $[e_1,s_2)$ is wasted and does not correspond to any component set. Adding a component set in this interval (e.g., by choosing a new $e_1'$ such that $s_1 \prec s_2 \prec e_1 \prec e_2$ and $s_1 \prec s_2 \prec e_1 \prec s_3$) does not reduce the number of feedback sequences since for two component sets $\mathcal{C} \subset \mathcal{C}'$ the corresponding set of FIS satisfy $\mathcal{F} \subset \mathcal{F}'$. 
%     \item We have $s_1 \prec s_2 \prec e_2 \prec s_3 $ and $s_1 \prec s_2 \prec e_2 \prec e_1$. 
% \end{itemize}




% First, we note that for the optimal set of

\proof
Assumption: the probability is nonzero over $[0,2\pi)$.
Consider a set of $b$ contiguous scanning beams $\mathcal{B}$ positioned on a circle. Let $\mathcal{C}$ denote the set of component beams generated by the set of scanning beams $\mathcal{B}$. 

First, we note that without loss of generality we can assume that set of starting and ending point of each scanning beam interval, i.e., \emph{end point markers}, are disjoint, which means there every starting point and ending point is unique. Suppose not; consider the ordered set of end point markers $x_1 \succ x_2 \succ \ldots \succ x_{2b}$ and assume that two consecutive points $x_i$ and $x_j$ (say $x_1$ and $x_2$ or $x_{2b}$ and $x_1$) are equal $x_i = x_j$ and we have $x_{i-1} \succ x_i \succ x_{j+1}$. Consider two cases: (i) At least one of the points $x_i$ and $x_j$ are an ending point. Let $x_j$ be an ending point. By moving it to point $x_j'$ such that $x_i \succ x_j' \succ x_{j+1}$, one can generate an extra component beams. (ii) Both $x_i$ and $x_j$ are an starting point. By moving $x_i$ to point $x_i'$ such that $x_{i-1} \succ x_i' \succ x_j$, one can generate an extra component beams. In either case (i) or case (ii), by adding a new component beam to the set $\mathcal{C}$, the cardinality of $\mathcal{C}^2$ cannot decrease. 

Hence, we can assume that in the maximal case of $\mathcal{C}$, its cardinality is exactly $2b$. In other words, there exist a $\mathcal{C}$ which is maximal, i.e., the cardinality of $\mathcal{C}^2$ is maximum. It can be easily verified that when considering $2b$ the component beams on the loop, the spawning sets of any two consecutive component beam differ only in one element.

%Second, consider the case that there are two \emph{singleton} in the set of component beams, i.e., two component beams of degree 1. In the following we will show that the set of component beam between these two intervals can be modified to form a tulip structure without deceasing the cardinality of the set of possible feedback sequences that is equal to $\mathcal{C}^2$.  

\emph{Claim 1}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| < |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-2$. One of the following four cases might have occurred, and in each case all three unions $A \cup A_n$, $A \cup A_{n-1}$, and $A \cup A_{n-2}$ are repeated in some other combinations and hence they do not generate a new spawning set in $(\mathcal{A} \cup A)^2$. We have (i) $A_{n-2} \supset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$ or $A_{n-1}$; (iii) $A_{n-2} \subset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A$ or $A_{n-2}$; (iv) $A_{n-2} \supset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A_n \cup A_{n-2}$. Hence, at most $n-3$ new subsets of the form $A_i \cup A, 1 \leq i \leq n-3$ and one new subset corresponding to the new subset $A$ are generated.

\emph{Claim 2}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| > |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-1$ or $|(\mathcal{A} \cup A)^2| \leq 2n$ . One of the following three cases might have occurred. We have (i) $A_{n-1} \subset A_{n} \subset A$ in which case $A \cup A_n = A$, $A \cup A_{n-1} = A$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_n = A$ and $A \cup A_{n-2} = A \cup A_{n-1}$; (iii) $\exist i, i \geq 1$ such that $A_i \subset A_{i+1} \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_i = A \cup A_{i+1}$ and $A \cup A_{n} = A$; (iv) $A_1 \supset A_2 \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$. Hence, for the first three cases at most $n-2$ new subsets of the form $A_i \cup A$ out of all subset of $A_i \cup A , 1 \leq i \leq n$ plus one new subset $A$ are generated. Otherwise, in case (iv) the possible different subsets are only in the form of $A_1, A_2, \ldots, A_n, A \cup A_1, A \cup A_2, \ldots, A \cup A_n$ which are 2n in total.

Let $F_n$ is the maximum number of elements in the $|(\mathcal{A})^2|$ where $|A| = n$. It can be directly checked for the small number of $n \leq 5$ that $F_1 = F_2 = F_3 = 1$, $F_4 = 5$, and $F_5 = 8$. Based on the results of claim 1 and 2, we can prove that $F_{n+2} \leq F_n + 2n - 2$, hence we have
\begin{align}
    \left\{ \begin{array}{ll}
        F_n \leq \frac{n(n-4)}{2}+5, & n = 2b, n \geq 4 \\
        F_n \leq \frac{(n+1)(n-5)}{2}+8, & n = 2b-1, n \geq 5 
    \end{array}
    \right.
\end{align}

\emph{Claim 3:} Now consider two adjacent but not overlapping subsets $\mathcal{A} = \{A_1, \ldots, A_n\}$ and $\mathcal{D} = \{D_1, \ldots, D_m\}$ of the $\mathcal{C}$ that partition $\mathcal{C}$ into two pieces. Hence, either pair $\{A_n, D_1\}$ and $\{D_m, A_1\}$ are adjacent. For the pair $\{A_n, D_1\}$, either we have $A_n \subset D_1$ or vice versa. There are at most $|\mathcal{A}| \times |\mathcal{D}|$ elements in the union-product $\mathcal{A} \times \mathcal{D}$, where we show that under some conditions there are 5 terms in vicinity of $\{A_n, D_1\}$ and another five terms in vicinity of $\{D_m, A_1\}$ are redundant, i.e., they either generated in two different product terms in $\mathcal{A} \times \mathcal{D}$ or they already belong to $\mathcal{A}^2$ or $\mathcal{D}^2$. First we prove that there are 5 redundant terms in vicinity of the pair $\{A_n, D_1\}$. The proof for the pair $\{D_m, A_1\}$ is similar. For the pair $\{A_n, D_1\}$, either we have $A_n \subset D_1$ or vice versa. Without loss of generality we can assume $A_n \subset D_1$ and the other case can be obtained through a symmetric argument.

Let $a = D_1 - A_n$. let $i$ be the smallest index such that $A_{n} \not \subset  D_{i}$ %$D_{i-1} \not \subset  D_{i}$ 
and $j$ be the smallest index for which $a \notin D_j$. We have (i) $A_n \cup D_1$ = $D_1 \cup D_1 \in \mathcal{D}^2$, (ii) $A_n \cup D_i = A_n \cup D_{i-1}$, i.e., they are redundant, and (iii) $A_n \cup D_{j-1} = D_1 \cup D_j \in \mathcal{D}^2$. Also, let $k$ be the largest index such that $A_n \not \subset A_k$. We have, (iv) $A_k \cup D_1 = A_{k+1} \cup D_1$, i.e., they are redundant, and (v) $A_k \cup D_{i-1} = A_{k+1} \cup D_i$, i.e., they are redundant. It can be easily verified that $i \neq n$, $j \neq n$, $k \neq 1$ and $i \neq j$, hence, the terms $A_n \cup D_1$, $A_n \cup D_i$, $A_n \cup D_j$, $A_k \cup D_{j-1}$, and $A_k \cup D_1$ are all different terms in $\mathcal{A} \times \mathcal{D}$. However, the existence of the indices $i, j, k$ is not Guaranteed, but if they exist there are total of 10 terms in $|\mathcal{A}| \times |\mathcal{D}|$ which are redundant and it completes the proof of claim 3. 

Now let us consider what happens if the index $i$ does not exist. This means that for all $D_i \in \mathcal{D}$ we have $A_n \subseteq D_i$

%Let $a = D_1 - A_n$. let $i$ be the smallest index such that $A_i \not \subset  A_{i-1}$ and $j$ be the smallest index for which $a \notin A_j$. We have (i) $A_n \cup D_1$ = $D_1 \cup D_1 \in \mathcal{D}^2$, (ii) $A_n \cup A_i = A_n \cup A_{i-1}$, i.e., they are redundant, and (iii) $A_n \cup A_{j-1} = D_1 \cup A_j \in \mathcal{D}^2$. Also, let $k$ be the largest index such that $A_n \not \subset D_k$. We have, (iv) $A_k \cup D_1 = A_{k+1} \cup D_1$, i.e., they are redundant, and (v) $A_k \cup A_{i-1} = A_{k+1} \cup A_i$, i.e., they are redundant. This completes the proof of claim 3. 

For the final step of the proof, we consider the set of spawning sets $\mathcal{C}$ with $2b$ elements. The statement of the theorem for small values of $b \leq 4$ can be verified directly. For $b \geq 5$, we consider an arbitrary partitioning of the loop into $2a \geq 4$ and $2(b-a) \geq 4$ elements, e.g., $A_1, A_2, \ldots, A_{2a}, D_1, D_2, \ldots, D_{2b-2a}$. Define $\mathcal{A} = \{A_1, \ldots, A_{2a}\}$ and $\mathcal{D} = \{D_1, \ldots, D_{2b-2a}\}$ where either $A_n \notsubset A_1$ or $A_1 \not subset A_n$ which follows from the fact that there are no single beam nor double beam loop in the maximal design (to add the proof). We have $\mathcal{C} = \mathcal{A} \cup \mathcal{D}$. Hence, we have $|\mathcal{C}^2| \leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|$. Since $\mathcal{A}$ has $2a$ elements and $\mathcal{D}$ has $2b-2a$ elements, we have $|\mathcal{A}^2| \leq 2a(a-2)+5$ and $|\mathcal{D}^2| \leq 2(b-a)(b-a-2)+5$. On the other hand $\mathcal{A} \times \mathcal{D} \leq 2a(2b-2a) - 10$. Hence 
\begin{align}
    |\mathcal{C}^2| &\leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|\\
    &\leq (2a(a-2)+5) + (2(b-a)(b-a-2)+5) \\
    &+ (2a(2b-2a) -10) \\
    &\leq 2b(b-2)
\end{align}

On the other hand we know that for Tulip structure we have $|\mathcal{C}^2| = 2b(b-2)$ which means that Tulip structure is a maximal or optimal structure.


% \emph{Claim 1}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| < |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-1$. One of the following two cases might have occurred. (i) $A_{n-1} = A_n - \{a_2\}$ and $A = A - \{a_1\}$, or (ii) $A_{n-1} = A_n \cup \{a\}$ and $A = A - \{a_1\}$ for some $a_1, a_2 \in A_n$, $a_1 \neq a_2$ and $a \notin A$. In either case $A \cup A_n$ and $A \cup A_{n-1}$ does not generate a new subset in $|(\mathcal{A} \cup A)^2|$ Hence, at most 
% n-2 new subset of the form $A_i \cup A, 1 \leq i \leq n-2$ and the new subset $A$ is generated.

% \emph{Claim 2}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| > |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-2$. One of the following four cases might have occurred. (i) $A_{n-2} = (A_n \cup \{a\}) - \{a_2\}$, $A_{n-1} = A_n - \{a_2\}$ and $A = A - \{a_1\}$, or (ii) $A_{n-2} = A_n - \{a_2, a_3\}$, $A_{n-1} = A_n - \{a_2\}$ and $A = A \cup  - \{a_1\}$, or (iii) $A_{n-2} = (A_n \cup \{a\}) - \{a_2\}$, $A_{n-1} = A_n -{a_2}$ and $A = A - {a_1}$, or (i) $A_{n-2} = A_n -{a_2}+{a}$, $A_{n-1} = A_n -{a_2}$ and $A = A - {a_1}$, or (iii) $A_{n-1} = A_n + {a}$ and $A = A - {a_1}$ for some $a_1, a_2 \in A_n$, $a_1 \neq a_2$ and $a \notin A$. In either case $A \cup A_n$ and $A \cup A_{n-1}$ does not generate a new subset in $|(\mathcal{A} \cup A)^2|$ Hence, at most 
% n-2 new subset of the form $A_i \cup A, 1 \leq i \leq n-2$ and the new subset $A$ is generated.

\begin{thm}
A set of scanning beams with flower design (defined earlier?) generates the maximal number of possible feedback sequences. For $p > 1$, flower design is the only?? maximal set?
\label{thm: flower}
\end{thm}



==> tulip_proof1.tex <==
\section{Problem Formulation}
\label{sec:problem}

THIS IS THE TULIP PROOF

\begin{defn}
A contiguous beam, say scanning beam, is denoted by its angular coverage interval (ACI). For example a beam $i$ is denoted as $[s_i,e_i)$ where $s_i$ is the starting point (angle) and $e_i$ is the ending point (angle). 
\label{defn: contiguous}
\end{defn}



\begin{defn}
A direction is defined on the azimuth angles, say, counter-clockwise. The ACI as well as the starting and the ending point of a beam is measured with respect to this direction. For example, one may have a beam starting at $3\pi/2$ and ending at $\pi/2$ which is represented as $[ 3 \pi /2, \pi/2)$.
\label{defn: loop}
\end{defn}

\begin{defn}
Consider a set of points $a_1, a_2, \ldots, a_n$, $n\geq3$ on a circle. For any three indices $1 \leq i, j, k \leq n$, we write $a_i \prec a_j \prec a_k$ (and read as  $a_i$ precedes $a_j$ precedes $a_k$) if by starting from point $a_i$ and moving in the defined direction (say counter clockwise) we first encounter $a_j$ and then encounter $a_k$ before reaching $a_i$ again. Equivalently, we write $a_k \succ a_j \succ a_i$ and read $a_k$ succeeds $a_j$ succeeds $a_i$. Please note that the precedence relation requires at least three points to be specified.
\label{defn: prec_succ}
\end{defn}


\begin{defn}
Consider $b$ beams and denote them by beam $i$, $i \in B$ where $B = {1, 2, \ldots, b}$ denotes the set of all possible beam. For a given subset $C \subset B$, we define a component beam $\omega_C$ as a beam (possibly comprised of an interval or a collection of intervals) where each differential arc of the beam contains all the beams in $C$ and does not contain any beam which is not in $C$. The set $C$ is called the \emph{spawning set} of $\omega_C$ and its cardinality is called the \emph{degree} of $\omega_C$. A component beam with spawning set $C$ may or may not exist, and if it exist we may refer to the component beam by its spawning set $C$.  We say a \emph{component beam has a beam $i$ in its intersection} if the beam $i$ belongs to its spawning set.
\label{defn:component}
\end{defn}

% \begin{defn}
% A component beam is always a subset of an intersection of scanning beams. The minimal number of beams for which the component beam is a subset of intersection of those beams is called the \emph{spawning set} and its cardinality is called the \emph{degree} of that component beam. We say a \emph{component beam has a beam $i$ in its intersection} if the beam $i$ belongs to its spawning set.
% \label{defn:degree}
% \end{defn}

\begin{defn} [NOT REQUIRED]
Consider a set of scanning beam as $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that without loss of generality $s_1 \prec s_2 \prec \ldots \prec s_b$. For any $i$ and $j$, if $s_i \prec s_j \prec e_j \prec e_i$ then we say beam $j$ is nested in beam $i$ and beam $i$ is the host of beam $j$. If beam $j$, $j>i$ is nested in beam $i$ and there is no other beam $k$, $j > k > i$ that is nested in $i$, we say the beam $j$ is the first nested beam in beam $i$.  
\label{defn:nested}
\end{defn}

\begin{defn}
We define the following operators and notations on spawning set. Let a spawning set (or equivalently a component beam) be denoted by capital letters $C, D, E, F, X, Y$, etc., and a set of spawning sets be represented by $\mathcal{C}, \mathcal{E}$, etc., e.g., $\mathcal{C} = \{C, D\}$, and $\mathcal{E} = \{E, F\}$. The union of two spawning set $C \cup D$ is denoted by $CD$. The cross product (or product or union product) of two sets of spawning sets $\mathcal{C}$ and $\mathcal{E}$ is denoted by $\mathcal{C} \times \mathcal{E}$ and is defined as a set that contains the union of any pair of sets such that one set belongs to the first and the other one belongs to the second set of spawning sets, i.e., $\mathcal{C} \times \mathcal{E} = \{X, X = X_1 X_2, X_1 \in \mathcal{C}, X_2 \in \mathcal{D}\}$. For example $\{C,D\} \times \{E,F\} = \{CE, CF, DE, DF\}$. The multiplication of the set of spawning sets $\mathcal{C}$ by itself may be represented as $\mathcal{C}^2 = \mathcal{C} \times \mathcal{C}$. The higher power $k > 2$ may be defined recursively as $\mathcal{C}^k = \mathcal{C}^{k-1} \times \mathcal{C}$.
\label{defn:product}
\end{defn}

\begin{defn} [NOT REQUIRED]
For a set of spawning sets $\mathcal{C}$ and an spawning set $D$ the \emph{back division} operator is defined as $\mathcal{C} \setminus D= \{X, DX \in \{D\} \times \mathcal{C}, D \cap X = \emptyset \}$.
\label{defn:back-division}
\end{defn}

If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $\setminus$ has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$

\begin{defn} 
For a set of spawning sets $\mathcal{C}$ and an spawning set $D$ the \emph{forward division} operator is defined as $\mathcal{C} / D= \{X, DX \in \mathcal{C} \}$.
\label{defn:forward-division}
\end{defn}

\begin{defn}[NOT REQUIRED]
For a set of spawning sets $\mathcal{C}$ and two spawning set $D$, $E$ the \emph{forward division} operator is defined as
$$\mathcal{C} / \{D,E\}= \{X, ((D-A)X \in \mathcal{C} \setminus E \wedge (E-A)X \in \mathcal{C} \setminus D) \lor$$
$$ (DEX \in \mathcal{C}), A = D \cap E  \}$$.
$$\mathcal{C} / \{D,E\}= \{X, (DX \in \mathcal{C} \setminus E \wedge EX \in \mathcal{C} \setminus D) \lor (DEX \in \mathcal{C} \setminus A)\}$$.
$$\mathcal{C} / \{D,E\}= \{X, (DX \in \mathcal{C} \setminus A \wedge EX \in \mathcal{C} \setminus A) \lor (DEX \in \mathcal{C} \setminus A), A = D \cap E \}$$.
\label{defn:forward-division2}
\end{defn}

If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $/$ had precedence on $\setminus$ which in turn has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$

\begin{properties}[NOT REQUIRED]
For a set of spawning sets $\mathcal{C}$ and a spawning sets $A$, $D$, $E$, $E \cap A \emptyset$, we have
\begin{align}
    \mathcal{C} \setminus AD = (\mathcal{C} \setminus A) \setminus D \\
%    |A \times \mathcal{C}| = |A \times \mathcal{C} \setminus A| \\    
    A \times \mathcal{C} = A \times \mathcal{C} \setminus A \\
    (A \times \mathcal{C}) \cap (AD \times \mathcal{C}) = A \times (\mathcal{C} - \mathcal{C} \setminus D) \\
    |(A \times \mathcal{C}) \cap (AD \times \mathcal{C})| \leq |\mathcal{C} - \mathcal{C} \setminus D| \\
    |AD \times \mathcal{C}| \leq |A \times \mathcal{C}| \\
    |A \times \mathcal{C}| = |\mathcal{C} \setminus A| \\
%    |\{A,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus E| - |(\mathcal{C} / A) \cap (\mathcal{C} / E) | \\
    |\{A,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus E| - |\mathcal{C} / \{D, E\}| \\
%    |\{A,AE\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus AE| - |(\mathcal{C} / AE) \cap (\mathcal{C} / E) | \\
    |\{A,D,E\} \times \mathcal{C}| = |\mathcal{C} \setminus A| + |\mathcal{C} \setminus D| + |\mathcal{C} \setminus E| \nonumber \\
    - |\mathcal{C} / \{A, D\}| - |\mathcal{C} / \{A, E\}| - |\mathcal{C} / \{D, E\}| \nonumber \\
    + |(\mathcal{C} / \{A, D\}) \cap (\mathcal{C} / \{A, E\}) \cap (\mathcal{C} / \{D, E\})| \\
     |\{A_i\}_{i \in [n]} \times \mathcal{C}| = \sum_{i=1}^n |\mathcal{C} \setminus A_i|  \nonumber \\
    - \sum_{s_2 \in S_2[n]} T(s_2) + \sum_{s_3 \in S_3[n]} |\cap_{s_2 \in s_3} T(s_2)| \nonumber \\
    - \sum_{s_4 \in S_4[n]} |\cap_{s_2 \in s_4} T(s_2)| + \ldots \\ 
    \mbox{where } S_k[n] = \{ \{i_1, \ldots, i_k\},  i_l \in [n] \nonumber \\
    \mbox{for } 1 \leq l \leq k, i_1 < i_2 < \ldots < i_k \} \nonumber \\
    \mbox{and } T(s_2) = \mathcal{C} / \{A_{i_1}, A_{i_2}\}, \mbox{for } s_2 = \{i_1, i_2\} \nonumber
\end{align}
\label{defn:division-properties}
\end{properties}

[NOT REQUIRED]The property 3 may be valid for the spawning sets of a single beam only and the extension may be different. I have to think about it more. The property 4 is derived from property 3.

\begin{defn}
A set of scanning beam has Tulip design if there exist an ordering of the beam in the form of $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that for every $i$ we have $s_i \prec e_{i-1} \prec s_{i+1} \prec e_i$ %$e_{i-1}, s_{i+1} \in (s_i,e_i)$.   
\label{defn:tulip}
\end{defn}

\begin{defn}
If a set of beams $B' \subset B, B = \{1, 2, \ldots, b\}$, is used for probing, the feedback sequence is a sequence of length $b$ with ternary values where the position $i$ corresponds to the feedback of beam $i$ and it is set to $1$, $0$ for positive and negative feedback, respectively. If the beam $i$ is not used for probing the position $i$ in feedback sequence is set to $x$. Corresponding to a feedback sequence, we define a \emph{feedback index set (FIS)} which contains the indices of the beams for which a positive feedback is received. The cardinality of FIS for a feedback sequence is defined as its degree.
\label{defn:FBS}
\end{defn}


\begin{lemma}
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 1$ path.
\label{lemma:Tulip_1}
\end{lemma}

\proof
The proof relies on the fact that $b$ contiguous beams have total of $2b$ starting and ending points and hence can generate at most $2b$ component beams. On the other hand for $p=1$ a feedback sequence is valid only and only if the set of the indices of the beam with positive feedback corresponds to an spawning set of a component beam that is realized by the set of scanning beams. Since there are at most $2b$ component beam, there is only $2b$ possible feedback sequences and Tulip design already provides $2b$ component beams. We note that the Tulip structure is not the only optimal design for $p=1$.

\begin{lemma}
For a channel with $p=2$ paths, a set of scanning beams with Tulip design generates $1, 3, 7$, and  $15$ feedback sequences for $b = 1, 2, 3$, and 4 beams, respectively, and generates $2b(b-2)$ feedback sequences for $b > 4$ beams. 
\label{lemma:Tulip_2_count}
\end{lemma}

\proof
The proof is simply follows from a direct counting argument.
There are $b$ component beams of degree 1 with spawning sets $\{1\}, \{2\}, \ldots, \{b\}$ that are directly part of the Tulip design. For $b>1$, there are $b \choose 2$ feedback sequences of degree 2 corresponding to the beam index sets $\{12\}, \{13\}, \ldots, \{1b\}, \{23\}, \{24\}, \ldots, \{2b\}, \ldots, \{(b-1)b\}$. A degree 2 feedback sequence corresponding to an index set $\{ij\}$ can be generated by selecting path 1 and path 2 inside the component beams $\{i\}$ and $\{j\}$, respectively. For $b > 2$, a feedback sequence of degree 3 may be generated by selecting a path in a component beam of degree 2 and a path in a component beam of degree $1$. In the following consider the indices of the beam in mod $b$. In other words, the beam $b+1$ is the same as beam $1$. There are total of $b(b-3)$ feedback sequences of type $i(i+1)k$. Consider the set $C_i = \{ i(i+1)k, k \neq i, k \neq (i+1)\}$. There are $b$ sets $C_i, i = 1, 2, \ldots, b$, and each set $C_i$ has $b-2$ distinct feedback sequences and there are exactly $b$ feedback sequences of the form $i(i+1)(i+2)$ which appear in all sets 
$C_i, i = 1, 2, \ldots, b$ exactly twice. Hence the union $\cup_{i \on B} C_i$ contains exactly $b(b-3)$ distinct feedback sequences. Similarly, for $b>4$, it can be argued that there are exactly $b(b-3)/2$ degree 4 feedback sequences of type $i(i+1)j(j+1)$, $i+1 \succ j$, $j+1 \succ i$ that are generated by having one path in the component beam $i(i+1)$ and another in the component beam $j(j+1)$. For $b=4$, there is only one feedback sequence $1234$ that is generated by having one path in component beam $12$ and one path in component beam $34$. Summing all the feedback sequences of degree 1 to degree 4 proves the statement of the lemma.

\begin{lemma} [NOT REQUIRED]
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 2$ path, for an arbitrary distribution of channel AoD that is nonzero on $[0, 2 \pi)$
\label{lemma:Tulip_2}
\end{lemma}

\proof
Lemma~\ref{lemma:Tulip_1} proves the optimality of Tulip design for a channel with single path, i.e., $p=1$. Lemma~\ref{lemma:Tulip_2}, extends this optimality to the case of $p=2$, however, the proof is considerably more involved. 

Here, we first provide the sketch of the proof and then formally get into the details. Lemma~\ref{lemma:Tulip_2_count}, counts the number of feedback sequences that is generated by Tulip design. It is relatively easy to check for small numbers of $b \leq 5$ that no other set of scanning beams can generate more number of feedback sequences as Tulip design. For the case of $b>5$, we use induction to prove the lemma. For each step of the induction for $b+1$ beams, we select a beam and remove it. The resulting structure cannot generate more than $2b(b-2)$ feedback sequences per induction assumption. We show that adding the $b+1$ beam back to the previous structure cannot add more than $4b-2$ new feedback sequences. Hence, any structure with $b+1$ beams can generate at most $2b(b-2) + (4b - 2) = 2(b^2-2b+2b-1) = 2(b+1)(b-1) = 2(b+1)((b+1)-2)$ which is already achievable with Tulip structure. 

To prove the induction step for $b+1$ beams, we assume that we have an structure that is generating the maximum number of feedback sequences. First, we note that we can assume that the set of points $P$ consisting the starting points and ending points of each beam has exactly $2b$ points. Otherwise, if two points coincides, one can generate a new sets of beams by slightly moving one of the points. For such new beams the number of feedback sequences would not be less. Second, we prove that there is no beam that is nested in all other beams. In other words, if there is a beam where its starting point and ending point are immediately succeeding in the loop that consists of all the point of $P$ and there is no other points in $P$ that lie in between the staring an ending point of this beam. Suppose not, then by removing this beam the resulting number of feedback sequences is not more than $2b(b-2)$. By adding this $b+1$ beam back to the structure, one cannot generate more than $2b$ new feedback sequences, hence it is resulting less than $2(b+1)((b+1)-2)$ feedback sequences and it contradict the assumption that this structure generates the maximum number of feedback sequences.

Third, consider the case that the starting and the ending point of the beam $b+1$ is within two different component beams of the first $b$ beams. Let $C_b$, and $C_{b+1}$ denotes the set of component beams for the first $b$ beam and all $b+1$ beams, respectively. Assume the component beams in $C_b$ are denoted by $A_i$, i.e., $C_b = \{ A_1, A_2, \ldots, A_{2b}\}$. Hence, without loss of generality, there exist some $i$ and $j$ such that $C_{b+1} = (C_b - \{A_{i+1}, \ldots, A_(j-1)\}) \cup \{ (b+1)A_i, (b+1)A_{i+1}, \ldots, (b+1)A_j\}$, where $i$ and $j$ are the indices of the component beams where the starting and ending points of the beam $b+1$ fall within them.

The sets of FIS $F_b$ and $F_{b+1}$ for the first $b$ beams and all $b+1$ beams and $p=2$ is obtained as $F_b = C_b \times C_b$ and $F_{b+1} = C_{b+1} \times C_{b+1}$, respectively. We have
\begin{align}
    F_{b+1} &= \{A_k A_l\}_{k \in S, l \in S} \cup \{(b+1) A_k A_l\}_{k \in T, l \in T} \\
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in T} \\  
    &= \{A_k A_l\}_{k \in S, l \in S} \\
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in V} \\ 
    &\cup \{((b+1) A_k A_l\}_{k \in S, l \in U} \\
    &\cup \{(b+1) A_k A_l\}_{k \in U, l \in V} \\
    &\cup \{(b+1) A_k A_l\}_{k \in U, l \in U} 
    ,\mbox{and}\\
    F_{b} &= \{A_k A_l\}_{k \in B, l \in B} \\
    &= \{A_k A_l\}_{k \in S, l \in S} \\ 
    &\cup \{A_k A_l\}_{k \in S, l \in U} \\
    &\cup \{(A_k A_l\}_{k \in U, l \in U} 
\end{align}
where $S = \{1, 2, \ldots, i\} \cup \{j, j+1, b\}$ and $T = \{i, i+1, \ldots, j\}$, $U = \{i+1, i+2 \ldots, j-1\}$, $V = \{i, j\}$. I did not write the rest of the proof.

\begin{lemma}[NOT REQUIRED]
We say that there is a loop in the set of scanning beams, if there exist two beams $i$ and $j$ denoted by $[s_i,e_i)$ and $[s_j,e_j)$, respectively, such that $s_j \prec e_i \prec s_i \prec e_j$. If there is a loop in the set of scanning beams, it is always possible to open the loop by exchanging the beams $i$ and $j$ with two new beams that are not forming a loop such that as a result of opening the loop the number of feedback sequences is not decreased. 
\label{lemma: loop-free}
\end{lemma}

\proof
Define the following for intervals: $A = [s_j, e_i)$, $B = [e_i, s_i)$, $C = [s_i, e_j)$, $D = [e_j, s_i)$. WLOG, assume $i = 1$ and $j = 2$. Obviously, each component beam belong to at least one of these four sets. A component beam that belongs to set $A$ or $C$ has at least beam 1 and 2 in its intersection. Consider the component beam $\omega_{12}$. There are four cases: (i) $\omega_{12} \subset A$ and $\omega_{12} \subset C$, (ii) $\omega_{12} \not \subset A$ and $\omega_{12} \not \subset C$, (iii) $\omega_{12} \not \subset A$ and $\omega_{12} \subset C$, (iv) $\omega_{12} \subset A$ and $\omega_{12} \not \subset C$. For the case (i) to (iii) we set $E = A$ and for the case (iv) we set $E = C$. By removing the interval $E$ from both beams we generate two new beams with ACIs $[s_i,e_i)-E$ and $[s_j,e_j)-E$ that are not forming a loop. It remains to verify that the number of possible feedback sequences for the new beam set is not decreased. Since the old and new beam set only differ in interval $E$, any feedback sequence (FS) that is generated without a path in $E$ using old beam set can be generated by the new beam set as well. Now consider the case that there is still one path in $E$. Let $F$ denote the indices of the beams for a feedback sequence generated by a given set of paths including one path in $E$. For the old beam set, we always have $\{1,2\} \subset F$ and we can define $F' = F - \{1,2\}$. For the new set depending on where the paths outside $E$ are the indices of the beams for the feedback sequence for the new set is given by either $F'$, $F' \cup \{1\}$, $F' \cup \{2\}$, or $F' \cup \{1,2\}$ which are all different.


\begin{lemma}[NOT REQUIRED]
For a set of scanning beam $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ where $s_1 \prec s_2 \prec \ldots \prec s_b$, if the beam $j$ is the first nested beam in beam $i$, then exchanging the beam $i$ and $j$ with the two new beams $[s_i,e_j)$ and $[s_j, e_i)$, the number of possible feedback sequences is not decreased. 
\label{lemma: nested}
\end{lemma}

\proof


\begin{lemma}[NOT REQUIRED]
There exists an algorithm which can remove all possible nested beams to generate an un-nested set of scanning beams such that for the resulting scanning beams the number of possible feedback sequences is not decreased.
\label{lemma: termination}
\end{lemma}

\proof 
Define the ACIs of the set of scanning beams as $A_1, A_2, \ldots, A_b$ where $A_i = [s_i, e_i)$ and $s_1 \prec s_2 \prec \ldots \prec s_b$.
Consider the following algorithm. For $k = 1:b$, For $l = 1:k-1$, If $A_k$ is nested in $A_l$, exchange $e_k$ and $e_l$, endif, endfor, endfor. It can be easily verified that at the end of this algorithm, there is no nested beam. On the other hand, since each step of the algorithm uses the exchange of the end points of a nested beam with its parent (define parent of the nested beam), hence, using lemma~\ref{}, the number of possible feedback sequence is not decreased in each step and hence it is not decreased overall.

\proof
Consider any ordered


\begin{lemma}[NOT REQUIRED]
For an un-nested set of scanning beams, if there exists a component beam of degree three or more, there exist a new set of scanning beams with reduced degree for the same component beam for which the number of possible feedback sequences is not decreased.
\label{lemma:un-nested}
\end{lemma}

\begin{thm} [NOT REQUIRED: REVISED THEOREM STATEMENT BELOW]
The most distinguishable set, i.e., the set with the largest possible size, may be obtained through Tulip design defined by a set of single span SBs $\mathcal{B}=\left\{\Phi_{i}\right\}, i \in[b]$, where each beam may only have intersection with its adjacent beams with the exception of $\Phi_{1}$ and $\Phi_{b}$ for which the intersection might be nonempty. This means $\Phi_{i} \cap \Phi_{j}=\varnothing, 1<$ $|i-j|<b$
\end{thm}

% Some attempt
% \proof
% Lemma~\ref{lemma:Tulip_1} proves the statement of the theorem for the case of the channel with $p=1$ path. Here, we provide the proof for the case of $p>1$. We note that the set FIS $\mathcal{F}$ for the channel with $p$ path is obtained as $F = \mathcal{C}^p$ where $\mathcal{C}$ is the set of spawning set of all component beams.  

% Consider a set of scanning beams and select an arbitrary scanning beam and name it beam 1. Then select the other beams such that for the set of scanning beams $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ we have $s_1 \prec s_2 \prec \ldots \prec s_b$. 

% One of the following cases may occur.
% \begin{itemize}
%     \item We have $s_1 \prec e_1 \prec s_2$. In this case the arc $[e_1,s_2)$ is wasted and does not correspond to any component set. Adding a component set in this interval (e.g., by choosing a new $e_1'$ such that $s_1 \prec s_2 \prec e_1 \prec e_2$ and $s_1 \prec s_2 \prec e_1 \prec s_3$) does not reduce the number of feedback sequences since for two component sets $\mathcal{C} \subset \mathcal{C}'$ the corresponding set of FIS satisfy $\mathcal{F} \subset \mathcal{F}'$. 
%     \item We have $s_1 \prec s_2 \prec e_2 \prec s_3 $ and $s_1 \prec s_2 \prec e_2 \prec e_1$. 
% \end{itemize}




% First, we note that for the optimal set of

% \begin{thm} [REVISED THEOREM STATEMENT BELOW]
% If the probability of the paths is nonzero over $[0,2\pi)$, the most distinguishable set, i.e., the set with the largest possible size, of feedback sequences may be obtained through Tulip design.
% \end{thm}

\begin{lemma}
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 2$ path, for an arbitrary distribution of channel AoD that is nonzero on $[0, 2 \pi)$
\label{lemma:Tulip_2}
\end{lemma}

\proof
Lemma~\ref{lemma:Tulip_1} proves the optimality of Tulip design for a channel with single path, i.e., $p=1$. Lemma~\ref{lemma:Tulip_2}, extends this optimality to the case of $p=2$, however, the proof is considerably more involved. 

Here, we first provide the sketch of the proof and then formally get into the details. Lemma~\ref{lemma:Tulip_2_count}, counts the number of feedback sequences that is generated by Tulip design. It is relatively easy to check for small numbers of $b \leq 5$ that no other set of scanning beams can generate more number of feedback sequences as Tulip design. For the case of $b>5$, we prove the theorem by using the following steps.

Consider a set of $b$ contiguous scanning beams $\mathcal{B}$ positioned on a circle. Let $\mathcal{C}$ denote the set of component beams generated by the set of scanning beams $\mathcal{B}$. 

First, we note that without loss of generality we can assume that set of starting and ending point of each scanning beam interval, i.e., \emph{end point markers}, are disjoint, which means that every starting point and ending point is unique. Suppose not; consider the ordered set of end point markers $x_1 \succ x_2 \succ \ldots \succ x_{2b}$ and assume that two consecutive points $x_i$ and $x_j$ (say $x_1$ and $x_2$ or $x_{2b}$ and $x_1$) are equal $x_i = x_j$ and we have $x_{i-1} \succ x_i \succ x_{j+1}$. Consider two cases: (i) At least one of the points $x_i$ and $x_j$ are an ending point. Let $x_j$ be an ending point. By moving it to point $x_j'$ such that $x_i \succ x_j' \succ x_{j+1}$, one can generate an extra component beams. (ii) Both $x_i$ and $x_j$ are an starting point. By moving $x_i$ to point $x_i'$ such that $x_{i-1} \succ x_i' \succ x_j$, one can generate an extra component beams. In either case (i) or case (ii), by adding a new component beam to the set $\mathcal{C}$, the cardinality of $\mathcal{C}^2$ cannot decrease. 

Hence, we can assume that in the maximal case of $\mathcal{C}$, its cardinality is exactly $2b$. In other words, there exist a $\mathcal{C}$ which is maximal, i.e., $|\mathcal{C}^2|$ is maximum when $|\mathcal{C}| = 2b$. It can be easily verified that when considering $2b$ the component beams on the loop, the spawning sets of any two consecutive component beam $C_i$ and $C_{i+1}$ differ only in one element which means that (i) either $C_i \subset C_{i+1}$ or $C_i \supset C_{i+1}$ and (ii) $||C_i| - |C_{i+1}|| = 1$.

\emph{Claim 1}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| < |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-2$. One of the following four cases might have occurred, and in each case all three unions $A \cup A_n$, $A \cup A_{n-1}$, and $A \cup A_{n-2}$ are repeated in some other combinations and hence they do not generate a new spawning set in $(\mathcal{A} \cup A)^2$. We have (i) $A_{n-2} \supset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$ or $A_{n-1}$; (iii) $A_{n-2} \subset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A$ or $A_{n-2}$; (iv) $A_{n-2} \supset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A_n \cup A_{n-2}$. Hence, at most $n-3$ new subsets of the form $A_i \cup A, 1 \leq i \leq n-3$ and one new subset corresponding to the new subset $A$ are generated.

\emph{Claim 2}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| > |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-1$ or $|(\mathcal{A} \cup A)^2| \leq 2n$ . One of the following three cases might have occurred. We have (i) $A_{n-1} \subset A_{n} \subset A$ in which case $A \cup A_n = A$, $A \cup A_{n-1} = A$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_n = A$ and $A \cup A_{n-2} = A \cup A_{n-1}$; (iii) $\exist i, i \geq 1$ such that $A_i \subset A_{i+1} \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_i = A \cup A_{i+1}$ and $A \cup A_{n} = A$; (iv) $A_1 \supset A_2 \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$. Hence, for the first three cases at most $n-2$ new subsets of the form $A_i \cup A$ out of all subset of $A_i \cup A , 1 \leq i \leq n$ plus one new subset $A$ are generated. Otherwise, in case (iv) the possible different subsets are only in the form of $A_1, A_2, \ldots, A_n, A \cup A_1, A \cup A_2, \ldots, A \cup A_n$ which are 2n in total.

\emph{Claim 3:} Let $F_n$ is the maximum number of elements in the $|(\mathcal{A})^2|$ where $|A| = n$. It can be directly checked for the small number of $n \leq 5$ that $F_1 = F_2 = F_3 = 1$, $F_4 = 5$, and $F_5 = 8$. Based on the results of claim 1 and 2, we can prove that $F_{n+2} \leq F_n + 2n - 2$, hence we have
\begin{align}
    \left\{ \begin{array}{ll}
        F_n \leq \frac{n(n-4)}{2}+5, & n = 2b, n \geq 4 \\
        F_n \leq \frac{(n+1)(n-5)}{2}+8, & n = 2b-1, n \geq 5 
    \end{array}
    \right.
\end{align}

% Now consider two adjacent but not overlapping subsets $\mathcal{A} = \{A_1, \ldots, A_n\}$ and $\mathcal{D} = \{D_1, \ldots, D_m\}$ of the $\mathcal{C}$ that partition $\mathcal{C}$ into two pieces such that the pair $\{A_n, D_1\}$ (and $\{D_m, A_1\}$) are adjacent. There are at most $|\mathcal{A}| \times |\mathcal{D}|$ elements in the union-product $\mathcal{A} \times \mathcal{D}$, where we show that under some conditions there are 5 terms in vicinity of $\{A_n, D_1\}$ and another five terms in vicinity of $\{D_m, A_1\}$ are redundant, i.e., they either generated in two different product terms in $\mathcal{A} \times \mathcal{D}$ or they already belong to $\mathcal{A}^2$ or $\mathcal{D}^2$. First we prove that there are 5 redundant terms in vicinity of the pair $\{A_n, D_1\}$. The proof for the pair $\{D_m, A_1\}$ is similar. For the pair $\{A_n, D_1\}$, either we have $A_n \subset D_1$ or vice versa. Without loss of generality we can assume $A_n \subset D_1$ and the other case can be obtained through a symmetric argument.

% Now consider two adjacent but not overlapping subsets $\mathcal{A} = \{A_1, \ldots, A_n\}$ and $\mathcal{D} = \{D_1, \ldots, D_m\}$ of the $\mathcal{C}$ that partition $\mathcal{C}$ into two pieces. Hence, either pair $\{A_n, D_1\}$ and $\{D_m, A_1\}$ are adjacent. For the pair $\{A_n, D_1\}$, either we have $A_n \subset D_1$ or vice versa. We have
% \begin{align}
%     |\mathcal{C}^2| &\leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|
% \end{align}

\emph{Claim 4:} Let $\mathcal{A}_i = \{A \in \mathcal{C}, i \in A\}$ and $n_i = |\mathcal{A}_i|$. Obviously the set of component beams in $\mathcal{A}_i= \{A_1, A_2, \ldots, A_{n_i}\}$ are sequentially in order on the loop. Let $n$ be the maximum value of $n_i$ and correspondingly $\mathcal{A} = \mathcal{A}_i$ and $\mathcal{D} = \mathcal{C} - \mathcal{A}_i$. Assume the elements of $\mathcal{A} = \{A_1, \ldots, A_n\}$ and $\mathcal{D} = \{D_1, \ldots, D_m\}$ are in order on the loop such that $D_1$ and $D_m$ are the neighbors of $A_n$, $A_1$, respectively. We have $n+m=2b$.
Since $D_m \subset A_1$ and for the $i$ which maximizes $n_i$ we have $i \in A_1$ but $i \notin D_m$, hence $D_m \subset A_1$. Similarly we have and $D_1 \subset A_{n_i}$, which means that for all $k = 1, 2, \ldots, n_i$, we have $D_m A_i = A_1 A_i$ and $D_1 A_i = A_{n_i} A_i$. This means that there are $2n_i$ elements in $\mathcal{A} \times \mathcal{D}$ which is in common with elements in $\mathcal{A}^2$.
%Let $E_i$ and $F_i$ be the immediate component beam on the loop on the right and left hand side of $\mathcal{A}_i$, respectively. It can be verified that $E_i \subset A_1$ and $F_i \subset A_{n_i}$, which means that for all $k = 1, 2, \ldots, n_i$, we have $E_i A_i = A_1 A_i$ and $F_i A_i = A_{n_i} A_i$. Let $\mathcal{A} = \mathcal{A}_i$ and $\mathcal{D} = \mathcal{C} - \mathcal{A}_i$.  

If there is $n_i \geq 6$ then we have $|\mathcal{A} \times \mathcal{D}| \leq n_i * (2b-n_i) - 2 * n_i$ and for even $n_i$ we have
\begin{align}
    |\mathcal{C}^2| &\leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|\\
    &\leq (\frac{(n_i)(n_i - 4)}{2}+5) + (\frac{(2b-n_i)(2b-n_i - 4)}{2}+5) \nonumber \\
    &+ (n_i * (2b-n_i) - 2 * n_i) < 2b(b-2),
\end{align}
and for odd $n_i$ we have
\begin{align}
    |\mathcal{C}^2| & \leq (\frac{(n_i+1)(n_i - 5)}{2}+8) + \nonumber \\ 
    &(\frac{(2b-n_i+1)(2b-n_i - 5)}{2}+8)  \nonumber \\ 
    &+ (n_i * (2b-n_i) - 2 * n_i) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 6$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

\emph{Claim 5:} Next, assume that $n_i = 5$. We note that $D_1$ cannot be a subset $D_m$, otherwise there is a beam which is in at least $6$ consecutive component beams $A_n, D_1, D_2, \ldots, D_m$. Hence, we can find a minimum index $1 < k \leq m$ such that $D_1 \not \subset D_k$ for which we have $A_n D_k = A_n D_{k-1}$. Similarly, we have a minimum index $l$ such that $D_m \not \subset D_l$ for which we have $A_1 D_l = A_1 D_{l-1}$. 
On the other hand, there is a maximum index $1 \leq j < n$ such that $D_1 \not \subset A_j$ otherwise there is a common beam in at least 6 consecutive component beams $A_1, A_2, \ldots, A_n, D_1$. Hence we have $D_1 A_j = D_1 A_{j-1}$. Similarly there a minimal index $t$ such that $D_m \not \subset A_t$ otherwise there is a common beam in at least $6$ consecutive component beams $D_m, A_1, A_2, \ldots, A_n$. Hence we have $D_m A_t = D_m A_{t-1}$.
This means we have $|\mathcal{A} \times \mathcal{D}| \leq 5 * (2b-5) - 2 * 5 - 4$ and
\begin{align}
    |\mathcal{C}^2| & \leq (8) + (\frac{(2b-4)(2b- 10)}{2}+8)  \nonumber \\ 
    &+ (5 * (2b-5) - 14) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 5$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

\emph{Claim 6:} Next, assume that $n_i = 4$. This case is very similar to the Claim 5 for $n_i = 5$ which the exception that we use the formula of $F_n$ for the even $n$. We note that $D_1$ cannot be a subset $D_m$, otherwise there is a beam which is in at least $5$ consecutive component beams $A_n, D_1, D_2, \ldots, D_m$. Hence, we can find a minimum index $1 < k \leq m$ such that $D_1 \not \subset D_k$ for which we have $A_n D_k = A_n D_{k-1}$. Similarly, we have a minimum index $l$ such that $D_m \not \subset D_l$ for which we have $A_1 D_l = A_1 D_{l-1}$. 
On the other hand, there is a maximum index $1 \leq j < n$ such that $D_1 \not \subset A_j$ otherwise there is a common beam in the at least $5$ consecutive component beams $A_1, A_2, \ldots, A_n, D_1$. Hence we have $D_1 A_j = D_1 A_{j-1}$. Similarly there a minimal index $t$ such that $D_m \not \subset A_t$ otherwise there is a common beam in at least $5$ consecutive component beams $D_m, A_1, A_2, \ldots, A_n$. Hence we have $D_m A_t = D_m A_{t-1}$.
This means we have $|\mathcal{A} \times \mathcal{D}| \leq 4 * (2b-4) - 2 * 4 - 4$ and
\begin{align}
    |\mathcal{C}^2| & \leq (5) + (\frac{(2b-4)(2b-8)}{2}+5)  \nonumber \\ 
    &+ (4 * (2b-4) - 12) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 4$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

On the one hand, the max $n_i$ is less than or equal to 3. On the other hand for all $C_i$ in $\mathcal{C}$, $|C_i| \geq 1$ and for every two consecutive $C_i$ and $C_{i+1}$ we have $|C_i| = |C_{i+1}| \geq 3$. Hence, 
$$\sum_{i=1}^{b} n_i = \sum_{i=1}^{2b} |C_i| >= 3b$$
which means that all $n_i$ have to be equal to 3. This means that Tulip structure is maximal and indeed the unique optimal solution.


% There are at most $|\mathcal{A}| \times |\mathcal{D}|$ elements in the union-product $\mathcal{A} \times \mathcal{D}$, where we show that under some conditions there are 5 terms in vicinity of $\{A_n, D_1\}$ and another five terms in vicinity of $\{D_m, A_1\}$ are redundant, i.e., they either generated in two different product terms in $\mathcal{A} \times \mathcal{D}$ or they already belong to $\mathcal{A}^2$ or $\mathcal{D}^2$. First we prove that there are 5 redundant terms in vicinity of the pair $\{A_n, D_1\}$. The proof for the pair $\{D_m, A_1\}$ is similar. For the pair $\{A_n, D_1\}$, either we have $A_n \subset D_1$ or vice versa. Without loss of generality we can assume $A_n \subset D_1$ and the other case can be obtained through a symmetric argument.

% Let $a = D_1 - A_n$. let $i$ be the smallest index such that $A_{n} \not \subset  D_{i}$ %$D_{i-1} \not \subset  D_{i}$ 
% and $j$ be the smallest index for which $a \notin D_j$. We have (i) $A_n \cup D_1$ = $D_1 \cup D_1 \in \mathcal{D}^2$, (ii) $A_n \cup D_i = A_n \cup D_{i-1}$, i.e., they are redundant, and (iii) $A_n \cup D_{j-1} = D_1 \cup D_j \in \mathcal{D}^2$. Also, let $k$ be the largest index such that $A_n \not \subset A_k$. We have, (iv) $A_k \cup D_1 = A_{k+1} \cup D_1$, i.e., they are redundant, and (v) $A_k \cup D_{i-1} = A_{k+1} \cup D_i$, i.e., they are redundant. It can be easily verified that $i \neq n$, $j \neq n$, $k \neq 1$ and $i \neq j$, hence, the terms $A_n \cup D_1$, $A_n \cup D_i$, $A_n \cup D_j$, $A_k \cup D_{j-1}$, and $A_k \cup D_1$ are all different terms in $\mathcal{A} \times \mathcal{D}$. However, the existence of the indices $i, j, k$ is not Guaranteed, but if they exist there are total of 10 terms in $|\mathcal{A}| \times |\mathcal{D}|$ which are redundant and it completes the proof of claim 3. 

% Now let us consider what happens if the index $i$ does not exist. This means that for all $D_i \in \mathcal{D}$ we have $A_n \subseteq D_i$

% %Let $a = D_1 - A_n$. let $i$ be the smallest index such that $A_i \not \subset  A_{i-1}$ and $j$ be the smallest index for which $a \notin A_j$. We have (i) $A_n \cup D_1$ = $D_1 \cup D_1 \in \mathcal{D}^2$, (ii) $A_n \cup A_i = A_n \cup A_{i-1}$, i.e., they are redundant, and (iii) $A_n \cup A_{j-1} = D_1 \cup A_j \in \mathcal{D}^2$. Also, let $k$ be the largest index such that $A_n \not \subset D_k$. We have, (iv) $A_k \cup D_1 = A_{k+1} \cup D_1$, i.e., they are redundant, and (v) $A_k \cup A_{i-1} = A_{k+1} \cup A_i$, i.e., they are redundant. This completes the proof of claim 3. 

% For the final step of the proof, we consider the set of spawning sets $\mathcal{C}$ with $2b$ elements. The statement of the theorem for small values of $b \leq 4$ can be verified directly. For $b \geq 5$, we consider an arbitrary partitioning of the loop into $2a \geq 4$ and $2(b-a) \geq 4$ elements, e.g., $A_1, A_2, \ldots, A_{2a}, D_1, D_2, \ldots, D_{2b-2a}$. Define $\mathcal{A} = \{A_1, \ldots, A_{2a}\}$ and $\mathcal{D} = \{D_1, \ldots, D_{2b-2a}\}$ where either $A_n \notsubset A_1$ or $A_1 \not subset A_n$ which follows from the fact that there are no single beam nor double beam loop in the maximal design (to add the proof). We have $\mathcal{C} = \mathcal{A} \cup \mathcal{D}$. Hence, we have $|\mathcal{C}^2| \leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|$. Since $\mathcal{A}$ has $2a$ elements and $\mathcal{D}$ has $2b-2a$ elements, we have $|\mathcal{A}^2| \leq 2a(a-2)+5$ and $|\mathcal{D}^2| \leq 2(b-a)(b-a-2)+5$. On the other hand $\mathcal{A} \times \mathcal{D} \leq 2a(2b-2a) - 10$. Hence 
% \begin{align}
%     |\mathcal{C}^2| &\leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|\\
%     &\leq (2a(a-2)+5) + (2(b-a)(b-a-2)+5) \\
%     &+ (2a(2b-2a) -10) \\
%     &\leq 2b(b-2)
% \end{align}

% On the other hand we know that for Tulip structure we have $|\mathcal{C}^2| = 2b(b-2)$ which means that Tulip structure is a maximal or optimal structure.


% \emph{Claim 1}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| < |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-1$. One of the following two cases might have occurred. (i) $A_{n-1} = A_n - \{a_2\}$ and $A = A - \{a_1\}$, or (ii) $A_{n-1} = A_n \cup \{a\}$ and $A = A - \{a_1\}$ for some $a_1, a_2 \in A_n$, $a_1 \neq a_2$ and $a \notin A$. In either case $A \cup A_n$ and $A \cup A_{n-1}$ does not generate a new subset in $|(\mathcal{A} \cup A)^2|$ Hence, at most 
% n-2 new subset of the form $A_i \cup A, 1 \leq i \leq n-2$ and the new subset $A$ is generated.

% \emph{Claim 2}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| > |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-2$. One of the following four cases might have occurred. (i) $A_{n-2} = (A_n \cup \{a\}) - \{a_2\}$, $A_{n-1} = A_n - \{a_2\}$ and $A = A - \{a_1\}$, or (ii) $A_{n-2} = A_n - \{a_2, a_3\}$, $A_{n-1} = A_n - \{a_2\}$ and $A = A \cup  - \{a_1\}$, or (iii) $A_{n-2} = (A_n \cup \{a\}) - \{a_2\}$, $A_{n-1} = A_n -{a_2}$ and $A = A - {a_1}$, or (i) $A_{n-2} = A_n -{a_2}+{a}$, $A_{n-1} = A_n -{a_2}$ and $A = A - {a_1}$, or (iii) $A_{n-1} = A_n + {a}$ and $A = A - {a_1}$ for some $a_1, a_2 \in A_n$, $a_1 \neq a_2$ and $a \notin A$. In either case $A \cup A_n$ and $A \cup A_{n-1}$ does not generate a new subset in $|(\mathcal{A} \cup A)^2|$ Hence, at most 
% n-2 new subset of the form $A_i \cup A, 1 \leq i \leq n-2$ and the new subset $A$ is generated.

\begin{thm}
A set of scanning beams with flower design (defined earlier?) generates the maximal number of possible feedback sequences. For $p > 1$, flower design is the only?? maximal set?
\label{thm: flower}
\end{thm}



==> tulip_proof2.tex <==
\section{Problem Formulation}
\label{sec:problem}

THIS IS THE TULIP PROOF

\begin{defn}
A contiguous beam, say scanning beam, is denoted by its angular coverage interval (ACI). For example a beam $i$ is denoted as $[s_i,e_i)$ where $s_i$ is the starting point (angle) and $e_i$ is the ending point (angle). 
\label{defn: contiguous}
\end{defn}



\begin{defn}
A direction is defined on the azimuth angles, say, counter-clockwise. The ACI as well as the starting and the ending point of a beam is measured with respect to this direction. For example, one may have a beam starting at $3\pi/2$ and ending at $\pi/2$ which is represented as $[ 3 \pi /2, \pi/2)$.
\label{defn: loop}
\end{defn}

\begin{defn}
Consider a set of points $a_1, a_2, \ldots, a_n$, $n\geq3$ on a circle. For any three indices $1 \leq i, j, k \leq n$, we write $a_i \prec a_j \prec a_k$ (and read as  $a_i$ precedes $a_j$ precedes $a_k$) if by starting from point $a_i$ and moving in the defined direction (say counter clockwise) we first encounter $a_j$ and then encounter $a_k$ before reaching $a_i$ again. Equivalently, we write $a_k \succ a_j \succ a_i$ and read $a_k$ succeeds $a_j$ succeeds $a_i$. Please note that the precedence relation requires at least three points to be specified.
\label{defn: prec_succ}
\end{defn}


\begin{defn}
Consider $b$ beams and denote them by beam $i$, $i \in B$ where $B = {1, 2, \ldots, b}$ denotes the set of all possible beam. For a given subset $C \subset B$, we define a component beam $\omega_C$ as a beam (possibly comprised of an interval or a collection of intervals) where each differential arc of the beam contains all the beams in $C$ and does not contain any beam which is not in $C$. The set $C$ is called the \emph{spawning set} of $\omega_C$ and its cardinality is called the \emph{degree} of $\omega_C$. A component beam with spawning set $C$ may or may not exist, and if it exist we may refer to the component beam by its spawning set $C$.  We say a \emph{component beam has a beam $i$ in its intersection} if the beam $i$ belongs to its spawning set.
\label{defn:component}
\end{defn}

\begin{defn}
We define the following operators and notations on spawning set. Let a spawning set (or equivalently a component beam) be denoted by capital letters $C, D, E, F, X, Y$, etc., and a set of spawning sets be represented by $\mathcal{C}, \mathcal{E}$, etc., e.g., $\mathcal{C} = \{C, D\}$, and $\mathcal{E} = \{E, F\}$. The union of two spawning set $C \cup D$ is denoted by $CD$. The cross product (or product or union product) of two sets of spawning sets $\mathcal{C}$ and $\mathcal{E}$ is denoted by $\mathcal{C} \times \mathcal{E}$ and is defined as a set that contains the union of any pair of sets such that one set belongs to the first and the other one belongs to the second set of spawning sets, i.e., $\mathcal{C} \times \mathcal{E} = \{X, X = X_1 X_2, X_1 \in \mathcal{C}, X_2 \in \mathcal{D}\}$. For example $\{C,D\} \times \{E,F\} = \{CE, CF, DE, DF\}$. The multiplication of the set of spawning sets $\mathcal{C}$ by itself may be represented as $\mathcal{C}^2 = \mathcal{C} \times \mathcal{C}$. The higher power $k > 2$ may be defined recursively as $\mathcal{C}^k = \mathcal{C}^{k-1} \times \mathcal{C}$.
\label{defn:product}
\end{defn}


If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $\setminus$ has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$

\begin{defn} 
For a set of spawning sets $\mathcal{C}$ and an spawning set $D$ the \emph{forward division} operator is defined as $\mathcal{C} / D= \{X, DX \in \mathcal{C} \}$.
\label{defn:forward-division}
\end{defn}


If a set of spawning sets $\mathcal{D}$ contains a single spawning set $C$ it may be represented by $C$ instead of $\mathcal{D}$. Similarly, if a spawning set contains a single beam $c$, i.e., $C = \{ c\}$ it may be directly represented by $c$ instead of $C$. The definition of the operators $\setminus$ and $\times$ is inherited for the spawning sets and beams as well. For example, we may write $C \times \mathcal{D}$ where in this expression $C$ is interpreted as a set of spawning set which contains a single spawning set $C$. We denote the set minus operation by $-$, i.e., $C - D = \{x, x \in C, x \notin D \}$. We assume that the operator $/$ had precedence on $\setminus$ which in turn has precedence on the operators $\times$, $\cup$, $\cap$, and $-$ , e.g., $C \times \mathcal{D} E = C \times (\mathcal{D} \setminus E)$



\begin{defn}
A set of scanning beam has Tulip design if there exist an ordering of the beam in the form of $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ such that for every $i$ we have $s_i \prec e_{i-1} \prec s_{i+1} \prec e_i$ %$e_{i-1}, s_{i+1} \in (s_i,e_i)$.   
\label{defn:tulip}
\end{defn}

\begin{defn}
If a set of beams $B' \subset B, B = \{1, 2, \ldots, b\}$, is used for probing, the feedback sequence is a sequence of length $b$ with ternary values where the position $i$ corresponds to the feedback of beam $i$ and it is set to $1$, $0$ for positive and negative feedback, respectively. If the beam $i$ is not used for probing the position $i$ in feedback sequence is set to $x$. Corresponding to a feedback sequence, we define a \emph{feedback index set (FIS)} which contains the indices of the beams for which a positive feedback is received. The cardinality of FIS for a feedback sequence is defined as its degree.
\label{defn:FBS}
\end{defn}


\begin{lemma}
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 1$ path.
\label{lemma:Tulip_1}
\end{lemma}

\proof
The proof relies on the fact that $b$ contiguous beams have total of $2b$ starting and ending points and hence can generate at most $2b$ component beams. On the other hand for $p=1$ a feedback sequence is valid only and only if the set of the indices of the beam with positive feedback corresponds to an spawning set of a component beam that is realized by the set of scanning beams. Since there are at most $2b$ component beam, there is only $2b$ possible feedback sequences and Tulip design already provides $2b$ component beams. We note that the Tulip structure is not the only optimal design for $p=1$.

\begin{lemma}
For a channel with $p=2$ paths, a set of scanning beams with Tulip design generates $1, 3, 7$, and  $15$ feedback sequences for $b = 1, 2, 3$, and 4 beams, respectively, and generates $2b(b-2)$ feedback sequences for $b > 4$ beams. 
\label{lemma:Tulip_2_count}
\end{lemma}

\proof
The proof is simply follows from a direct counting argument.
There are $b$ component beams of degree 1 with spawning sets $\{1\}, \{2\}, \ldots, \{b\}$ that are directly part of the Tulip design. For $b>1$, there are $b \choose 2$ feedback sequences of degree 2 corresponding to the beam index sets $\{12\}, \{13\}, \ldots, \{1b\}, \{23\}, \{24\}, \ldots, \{2b\}, \ldots, \{(b-1)b\}$. A degree 2 feedback sequence corresponding to an index set $\{ij\}$ can be generated by selecting path 1 and path 2 inside the component beams $\{i\}$ and $\{j\}$, respectively. For $b > 2$, a feedback sequence of degree 3 may be generated by selecting a path in a component beam of degree 2 and a path in a component beam of degree $1$. In the following consider the indices of the beam in mod $b$. In other words, the beam $b+1$ is the same as beam $1$. There are total of $b(b-3)$ feedback sequences of type $i(i+1)k$. Consider the set $C_i = \{ i(i+1)k, k \neq i, k \neq (i+1)\}$. There are $b$ sets $C_i, i = 1, 2, \ldots, b$, and each set $C_i$ has $b-2$ distinct feedback sequences and there are exactly $b$ feedback sequences of the form $i(i+1)(i+2)$ which appear in all sets 
$C_i, i = 1, 2, \ldots, b$ exactly twice. Hence the union $\cup_{i \on B} C_i$ contains exactly $b(b-3)$ distinct feedback sequences. Similarly, for $b>4$, it can be argued that there are exactly $b(b-3)/2$ degree 4 feedback sequences of type $i(i+1)j(j+1)$, $i+1 \succ j$, $j+1 \succ i$ that are generated by having one path in the component beam $i(i+1)$ and another in the component beam $j(j+1)$. For $b=4$, there is only one feedback sequence $1234$ that is generated by having one path in component beam $12$ and one path in component beam $34$. Summing all the feedback sequences of degree 1 to degree 4 proves the statement of the lemma.



\begin{lemma}[NOT REQUIRED]
For a set of scanning beam $\{[s_1,e_1),[s_2,e_2),\ldots,[s_b,e_b),\}$ where $s_1 \prec s_2 \prec \ldots \prec s_b$, if the beam $j$ is the first nested beam in beam $i$, then exchanging the beam $i$ and $j$ with the two new beams $[s_i,e_j)$ and $[s_j, e_i)$, the number of possible feedback sequences is not decreased. 
\label{lemma: nested}
\end{lemma}

\proof



\begin{lemma}
Among the set of contiguous scanning beams, a set of scanning beams with Tulip design generates the maximal number of possible feedback sequences for the channel with $p = 2$ path, for an arbitrary distribution of channel AoD that is nonzero on $[0, 2 \pi)$
\label{lemma:Tulip_2}
\end{lemma}

\proof
Lemma~\ref{lemma:Tulip_1} proves the optimality of Tulip design for a channel with single path, i.e., $p=1$. Lemma~\ref{lemma:Tulip_2}, extends this optimality to the case of $p=2$, however, the proof is considerably more involved. 

Here, we first provide the sketch of the proof and then formally get into the details. Lemma~\ref{lemma:Tulip_2_count}, counts the number of feedback sequences that is generated by Tulip design. It is relatively easy to check for small numbers of $b \leq 5$ that no other set of scanning beams can generate more number of feedback sequences as Tulip design. For the case of $b>5$, we prove the theorem by using the following steps.

Consider a set of $b$ contiguous scanning beams $\mathcal{B}$ positioned on a circle. Let $\mathcal{C}$ denote the set of component beams generated by the set of scanning beams $\mathcal{B}$. 

First, we note that without loss of generality we can assume that set of starting and ending point of each scanning beam interval, i.e., \emph{end point markers}, are disjoint, which means that every starting point and ending point is unique. Suppose not; consider the ordered set of end point markers $x_1 \succ x_2 \succ \ldots \succ x_{2b}$ and assume that two consecutive points $x_i$ and $x_j$ (say $x_1$ and $x_2$ or $x_{2b}$ and $x_1$) are equal $x_i = x_j$ and we have $x_{i-1} \succ x_i \succ x_{j+1}$. Consider two cases: (i) At least one of the points $x_i$ and $x_j$ are an ending point. Let $x_j$ be an ending point. By moving it to point $x_j'$ such that $x_i \succ x_j' \succ x_{j+1}$, one can generate an extra component beams. (ii) Both $x_i$ and $x_j$ are an starting point. By moving $x_i$ to point $x_i'$ such that $x_{i-1} \succ x_i' \succ x_j$, one can generate an extra component beams. In either case (i) or case (ii), by adding a new component beam to the set $\mathcal{C}$, the cardinality of $\mathcal{C}^2$ cannot decrease. 

Hence, we can assume that in the maximal case of $\mathcal{C}$, its cardinality is exactly $2b$. In other words, there exist a $\mathcal{C}$ which is maximal, i.e., $|\mathcal{C}^2|$ is maximum when $|\mathcal{C}| = 2b$. It can be easily verified that when considering $2b$ the component beams on the loop, the spawning sets of any two consecutive component beam $C_i$ and $C_{i+1}$ differ only in one element which means that (i) either $C_i \subset C_{i+1}$ or $C_i \supset C_{i+1}$ and (ii) $||C_i| - |C_{i+1}|| = 1$.

\emph{Claim 1}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| < |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-2$. One of the following four cases might have occurred, and in each case all three unions $A \cup A_n$, $A \cup A_{n-1}$, and $A \cup A_{n-2}$ are repeated in some other combinations and hence they do not generate a new spawning set in $(\mathcal{A} \cup A)^2$. We have (i) $A_{n-2} \supset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n-1}$, and $A \cup A_{n-2} = A_{n-2}$ or $A_{n-1}$; (iii) $A_{n-2} \subset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A$ or $A_{n-2}$; (iv) $A_{n-2} \supset A_{n-1} \subset A_{n} \supset A$ in which case $A \cup A_n = A_n$, $A \cup A_{n-1} = A_{n}$, and $A \cup A_{n-2} = A_n \cup A_{n-2}$. Hence, at most $n-3$ new subsets of the form $A_i \cup A, 1 \leq i \leq n-3$ and one new subset corresponding to the new subset $A$ are generated.

\emph{Claim 2}: Consider a subset $\mathcal{A} = \{A_1, \ldots, A_n\}$ of $n$ elements of the $\mathcal{C}$ that are adjacent in the loop. If we add a new spawning set $A$ to one end of the loop (without loss of generality assume to the right hand side of the loop), and $|A| > |A_n|$, then $|(\mathcal{A} \cup A)^2| \leq |\mathcal{A}^2| + n-1$ or $|(\mathcal{A} \cup A)^2| \leq 2n$ . One of the following three cases might have occurred. We have (i) $A_{n-1} \subset A_{n} \subset A$ in which case $A \cup A_n = A$, $A \cup A_{n-1} = A$; (ii) $A_{n-2} \subset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_n = A$ and $A \cup A_{n-2} = A \cup A_{n-1}$; (iii) $\exist i, i \geq 1$ such that $A_i \subset A_{i+1} \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$ in which case $A \cup A_i = A \cup A_{i+1}$ and $A \cup A_{n} = A$; (iv) $A_1 \supset A_2 \supset \ldots \supset A_{n-2} \supset A_{n-1} \supset A_{n} \subset A$. Hence, for the first three cases at most $n-2$ new subsets of the form $A_i \cup A$ out of all subset of $A_i \cup A , 1 \leq i \leq n$ plus one new subset $A$ are generated. Otherwise, in case (iv) the possible different subsets are only in the form of $A_1, A_2, \ldots, A_n, A \cup A_1, A \cup A_2, \ldots, A \cup A_n$ which are 2n in total.

\emph{Claim 3:} Let $F_n$ is the maximum number of elements in the $|(\mathcal{A})^2|$ where $|A| = n$. It can be directly checked for the small number of $n \leq 5$ that $F_1 = F_2 = F_3 = 1$, $F_4 = 5$, and $F_5 = 8$. Based on the results of claim 1 and 2, we can prove that $F_{n+2} \leq F_n + 2n - 2$, hence we have
\begin{align}
    \left\{ \begin{array}{ll}
        F_n \leq \frac{n(n-4)}{2}+5, & n = 2b, n \geq 4 \\
        F_n \leq \frac{(n+1)(n-5)}{2}+8, & n = 2b-1, n \geq 5 
    \end{array}
    \right.
\end{align}


\emph{Claim 4:} Let $\mathcal{A}_i = \{A \in \mathcal{C}, i \in A\}$ and $n_i = |\mathcal{A}_i|$. Obviously the set of component beams in $\mathcal{A}_i= \{A_1, A_2, \ldots, A_{n_i}\}$ are sequentially in order on the loop. Let $n$ be the maximum value of $n_i$ and correspondingly $\mathcal{A} = \mathcal{A}_i$ and $\mathcal{D} = \mathcal{C} - \mathcal{A}_i$. Assume the elements of $\mathcal{A} = \{A_1, \ldots, A_n\}$ and $\mathcal{D} = \{D_1, \ldots, D_m\}$ are in order on the loop such that $D_1$ and $D_m$ are the neighbors of $A_n$, $A_1$, respectively. We have $n+m=2b$.
Since $D_m \subset A_1$ and for the $i$ which maximizes $n_i$ we have $i \in A_1$ but $i \notin D_m$, hence $D_m \subset A_1$. Similarly we have and $D_1 \subset A_{n_i}$, which means that for all $k = 1, 2, \ldots, n_i$, we have $D_m A_i = A_1 A_i$ and $D_1 A_i = A_{n_i} A_i$. This means that there are $2n_i$ elements in $\mathcal{A} \times \mathcal{D}$ which is in common with elements in $\mathcal{A}^2$.


If there is $n_i \geq 6$ then we have $|\mathcal{A} \times \mathcal{D}| \leq n_i * (2b-n_i) - 2 * n_i$ and for even $n_i$ we have
\begin{align}
    |\mathcal{C}^2| &\leq |\mathcal{A}^2| + |\mathcal{D}^2| + |\mathcal{A} \times \mathcal{D}|\\
    &\leq (\frac{(n_i)(n_i - 4)}{2}+5) + (\frac{(2b-n_i)(2b-n_i - 4)}{2}+5) \nonumber \\
    &+ (n_i * (2b-n_i) - 2 * n_i) < 2b(b-2),
\end{align}
and for odd $n_i$ we have
\begin{align}
    |\mathcal{C}^2| & \leq (\frac{(n_i+1)(n_i - 5)}{2}+8) + \nonumber \\ 
    &(\frac{(2b-n_i+1)(2b-n_i - 5)}{2}+8)  \nonumber \\ 
    &+ (n_i * (2b-n_i) - 2 * n_i) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 6$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

\emph{Claim 5:} Next, assume that $n_i = 5$. We note that $D_1$ cannot be a subset $D_m$, otherwise there is a beam which is in at least $6$ consecutive component beams $A_n, D_1, D_2, \ldots, D_m$. Hence, we can find a minimum index $1 < k \leq m$ such that $D_1 \not \subset D_k$ for which we have $A_n D_k = A_n D_{k-1}$. Similarly, we have a minimum index $l$ such that $D_m \not \subset D_l$ for which we have $A_1 D_l = A_1 D_{l-1}$. 
On the other hand, there is a maximum index $1 \leq j < n$ such that $D_1 \not \subset A_j$ otherwise there is a common beam in at least 6 consecutive component beams $A_1, A_2, \ldots, A_n, D_1$. Hence we have $D_1 A_j = D_1 A_{j-1}$. Similarly there a minimal index $t$ such that $D_m \not \subset A_t$ otherwise there is a common beam in at least $6$ consecutive component beams $D_m, A_1, A_2, \ldots, A_n$. Hence we have $D_m A_t = D_m A_{t-1}$.
This means we have $|\mathcal{A} \times \mathcal{D}| \leq 5 * (2b-5) - 2 * 5 - 4$ and
\begin{align}
    |\mathcal{C}^2| & \leq (8) + (\frac{(2b-4)(2b- 10)}{2}+8)  \nonumber \\ 
    &+ (5 * (2b-5) - 14) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 5$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

\emph{Claim 6:} Next, assume that $n_i = 4$. This case is very similar to the Claim 5 for $n_i = 5$ which the exception that we use the formula of $F_n$ for the even $n$. We note that $D_1$ cannot be a subset $D_m$, otherwise there is a beam which is in at least $5$ consecutive component beams $A_n, D_1, D_2, \ldots, D_m$. Hence, we can find a minimum index $1 < k \leq m$ such that $D_1 \not \subset D_k$ for which we have $A_n D_k = A_n D_{k-1}$. Similarly, we have a minimum index $l$ such that $D_m \not \subset D_l$ for which we have $A_1 D_l = A_1 D_{l-1}$. 
On the other hand, there is a maximum index $1 \leq j < n$ such that $D_1 \not \subset A_j$ otherwise there is a common beam in the at least $5$ consecutive component beams $A_1, A_2, \ldots, A_n, D_1$. Hence we have $D_1 A_j = D_1 A_{j-1}$. Similarly there a minimal index $t$ such that $D_m \not \subset A_t$ otherwise there is a common beam in at least $5$ consecutive component beams $D_m, A_1, A_2, \ldots, A_n$. Hence we have $D_m A_t = D_m A_{t-1}$.
This means we have $|\mathcal{A} \times \mathcal{D}| \leq 4 * (2b-4) - 2 * 4 - 4$ and
\begin{align}
    |\mathcal{C}^2| & \leq (5) + (\frac{(2b-4)(2b-8)}{2}+5)  \nonumber \\ 
    &+ (4 * (2b-4) - 12) < 2b(b-2). 
\end{align}
Hence, the maximal design cannot have $n_i \geq 4$ since for Tulip structure $|\mathcal{C}^2| = 2b(b-2)$.

On the one hand, the max $n_i$ is less than or equal to 3. On the other hand for all $C_i$ in $\mathcal{C}$, $|C_i| \geq 1$ and for every two consecutive $C_i$ and $C_{i+1}$ we have $|C_i| = |C_{i+1}| \geq 3$. Hence, 
$$\sum_{i=1}^{b} n_i = \sum_{i=1}^{2b} |C_i| >= 3b$$
which means that all $n_i$ have to be equal to 3. This means that Tulip structure is maximal and indeed the unique optimal solution.



\begin{thm}
A set of scanning beams with flower design (defined earlier?) generates the maximal number of possible feedback sequences. For $p > 1$, flower design is the only?? maximal set?
\label{thm: flower}
\end{thm}


